DeepTake: Prediction of Driver Takeover Behavior using Multimodal Data

Automated vehicles promise a future where drivers can engage in non-driving tasks without hands on the steering wheels for a prolonged period. Nevertheless, automated vehicles may still need to occasionally hand the control back to drivers due to technology limitations and legal requirements. While some systems determine the need for driver takeover using driver context and road condition to initiate a takeover request, studies show that the driver may not react to it. We present DeepTake, a novel deep neural network-based framework that predicts multiple aspects of takeover behavior to ensure that the driver is able to safely take over the control when engaged in non-driving tasks. Using features from vehicle data, driver biometrics, and subjective measurements, DeepTake predicts the driver's intention, time, and quality of takeover. We evaluate DeepTake performance using multiple evaluation metrics. Results show that DeepTake reliably predicts the takeover intention, time, and quality, with an accuracy of 96%, 93%, and 83%, respectively. Results also indicate that DeepTake outperforms previous state-of-the-art methods on predicting driver takeover time and quality. Our findings have implications for the algorithm development of driver monitoring and state detection.

==> DeepTakeArxiv/Figures/Illustrative_figure.tex <==

 
 %%%%%%
\begin{figure*}[h!]
   \centering
   \includegraphics[ width=\columnwidth]{Figures/DeepTake-overview-revised.png}
   \caption{DeepTake uses data from multiple sources (pre-driving survey, vehicle data, non-driving related tasks~(NDRTs) information, and driver biometrics) and feeds the preprocessed extracted features into deep neural network models for the prediction of takeover intention, time and quality.}
   \label{fig:llustrative}
\end{figure*} 
%%%%%%

==> DeepTakeArxiv/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> DeepTakeArxiv/Sections/0-abstract.tex <==
Automated vehicles promise a future where drivers can engage in non-driving tasks without hands on the steering wheels for a prolonged period. Nevertheless, automated vehicles may still need to occasionally hand the control back to drivers due to technology limitations and legal requirements. While some systems determine the need for driver takeover using driver context and road condition to initiate a takeover request, studies show that the driver may not react to it. We present DeepTake, a novel deep neural network-based framework that predicts multiple aspects of takeover behavior to ensure that the driver is able to safely take over the control when engaged in non-driving tasks. Using features from vehicle data, driver biometrics, and subjective measurements, DeepTake predicts the driver's intention, time, and quality of takeover. We evaluate DeepTake performance using multiple evaluation metrics. Results show that DeepTake reliably predicts the takeover intention, time, and quality, with an accuracy of 96\%, 93\%, and 83\%, respectively. Results also indicate that DeepTake outperforms previous state-of-the-art methods on predicting driver takeover time and quality. Our findings have implications for the algorithm development of driver monitoring and state detection.


==> DeepTakeArxiv/Sections/1-intro.tex <==

The rapid development of autonomous driving technologies promis-es a future where drivers can take their hands off the steering wheels and instead engage in non-driving related tasks (NDRTs) such as reading or using mobile devices. Incorporating cameras, sensors,
global positioning systems~(GPS), adaptive cruise control, light detection and ranging, and advanced driver assistance systems, automated vehicles (AVs) can navigate automatically. In Level 3 of autonomy (i.e., conditionally automated driving), as defined by the Society of Automotive Engineers (SAE international~\cite{sae2018taxonomy}), the driver does not need to continuously monitor the driving environment. Nevertheless, due to current technology limitations and legal restrictions, AVs may still need to handover the control back to drivers occasionally (e.g., under challenging driving conditions beyond the automated systems' capabilities)~\cite{mccall2019taxonomy}.
In such cases, AVs would initiate takeover requests (TORs) and alert drivers via auditory, visual, or vibrotactile modalities~\cite{naujoks2014effect,wan2018effects,pakdamanian2018effect} so that the drivers can resume manual driving in a timely manner.
However, there are challenges in making drivers safely take over control. Drivers may need a longer time to shift their attention back to driving in some situations, such as when they have been involved in NDRTs for a prolonged time~\cite{zeeb2017steering} or when they are stressed or tired~\cite{feldhutter2018wake}.
Even if TORs are initiated with enough time for a driver to react, it does not guarantee that the driver will safely take over~\cite{mcdonald2019toward}. Besides, frequent alarms could startle and increase drivers' stress levels leading to detrimental user experience in AVs~\cite{pakdamanian2020toward, korber2018have, lee2020analysis}. These challenges denote the need for AVs to constantly monitor and predict driver behavior and adapt the systems accordingly to ensure a safe takeover. 

%\todo{state of the art, gaps, challenges}

The vast majority of prior work on driver takeover behavior has focused on the empirical analysis of high-level relationships between the factors influencing takeover time and quality (e.g., \cite{mok2017tunneled,zhang2019determinants,du2020examining,ebnali2019does}). 
More recently, the prediction of driver takeover behavior using machine learning approaches has been drawing increasing attention. 
However, only a few studies have focused on the prediction of either takeover time~\cite{lotz2018predicting,berghofer2018prediction} or takeover quality~\cite{braunagel2017ready,deo2019looking,du2020predicting,du2020predictingtake}; and their obtained accuracy results (ranging from 61\% to 79\%) are insufficient for the practical implementation of real-world applications.
This is partly due to the fact that takeover prediction involves a wide variety of factors (e.g., drivers' cognitive and physical states, vehicle states, and the contextual environment) that could influence drivers' takeover behavior~\cite{zeeb2015determines}. \par

In this paper on the other hand, we present a novel approach, named \textbf{DeepTake}, to address these challenges by providing reliable predictions of multiple aspects of takeover behavior.
\textbf{DeepTake} is a unified framework for the prediction of driver takeover behavior in three aspects:
(1) \emph{takeover intention} -- whether the driver would respond to a TOR;
(2) \emph{takeover time} -- how long it takes for the driver to resume manual driving after a TOR;
and (3) \emph{takeover quality} -- the quality of driver intervention after resuming manual control.
As illustrated in Figure~\ref{fig:llustrative}, DeepTake considers multimodal data from various sources, including driver's pre-driving survey response (e.g., gender, baseline of cognitive workload and stress levels), vehicle data (e.g., lane position, steering wheel angle, throttle/brake pedal angles), engagement in NDRTs, and driver biometrics (e.g., eye movement for detecting visual attention, heart rate and galvanic skin responses for the continuous monitoring of workload and stress levels). This data can easily be collected in AVs' driving environment. For instance, all of the driver biometrics utilized in DeepTake can be captured by wearable smartwatches and deployed eye-tracking systems. 
The multitude of sensing modalities and data sources offer complementary information for the accurate and highly reliable prediction of driver takeover behavior. 
DeepTake extracts meaningful features from the preprocessed multimodal data, and feeds them into deep neural network (DNN) models with mini-batch stochastic gradient descent.
We built and trained different DNN models (which have the same input and hidden layers, but different output layers and weights) for the prediction of takeover behavior: intention, time and quality. 
We validate DeepTake framework feasibility using data collected from a driving simulator study. Finally, we evaluate the performance of our DNN-based framework with six machine learning-based models on prediction of driver takeover behavior. The results show that DeepTake models significantly outperform six machine learning-based models in all predictions of takeover intention, time and quality.
Specifically, DeepTake achieves an accuracy of 96\% for the binary classification of takeover intention, 93\%, and 83\% accuracy for multi-class classification of takeover time and quality, respectively. These accuracy results also outperform results reported in the existing work.


The main contribution of this work is the development of DeepTake framework that predicts driver takeover intention, time and quality using vehicle data, driver biometrics and subjective measurements\footnote{DeepTake framework configurations, implementation details and code are available at \url{ https://github.com/erfpak7/DeepTake}}. The intersection between ubiquitous computing, sensing and emerging technologies offers promising avenues for DeepTake to integrate modalities into a novel human-centered framework to increase the robustness of drivers’ takeover behavior prediction.
We envision that DeepTake can be integrated into future AVs, such that the automated systems can make optimal decisions based on the predicted driver takeover behavior.
For example, if the predicted takeover time exceeds the duration that the vehicle can detect situations requiring TORs, or the predicted takeover quality is too low to respond to TORs, the automated systems can warn the driver to engage less with the NDRT. In other words, DeepTake facilitates drivers to be distracted as long as they can properly respond and safely maneuver the vehicle.
The reliable prediction of driver takeover behavior provided by DeepTake framework would not only improve the safety of AVs, but also improve drivers' user experience and productivity in AVs (e.g., drivers can focus on NDRTs without worrying about missing any TORs and potential tragic circumstances).
We believe that our work makes a step towards enabling NDRTs in automated driving, and helps HCI researchers and designers to create user interfaces and systems for AVs that adapt to the drivers’ context.
% system is that it can predict if a driver will be able to takeover when there’s a situation requiring the driver to do so and let the driver to be distracted as long as the driver can properly respond to the situation

==> DeepTakeArxiv/Sections/2-related-work.tex <==


We discuss prior work on the analysis of takeover time and quality, and position our work in the context of state-of-the-art takeover behavior prediction research. \par

%\todo{Takeover intention?}
\textbf{Takeover time.}
In this paper, we consider the \emph{takeover time} as the period of time from the initiation of TOR to the exact moment of the driver resuming manual control~(see Figure~\ref{fig:Scenario}), following the ISO standard definition in~\cite{iso21959}. 
Note that the same concept has also sometimes been named as takeover reaction time or response time in the literature (e.g., \cite{johns2016exploring,kim2017takeover,petermeijer2017driver,eriksson2017takeover}). The empirical literature defines a large variety of takeover time from a mean of 0.87s to brake~\cite{winter2016effects}, to an average of 19.8s to response to a countdown TOR~
\cite{politis2018evaluation} and 40s to stabilize the vehicle~\cite{merat2014transition}. This range is derived from influential factors impacting perception, cognitive processing, decision-making and resuming readiness~\cite{gold2016taking,zeeb2015determines}.
A meta-analysis of 129 studies by Zhang et al.~\cite{zhang2019determinants} found that a shorter takeover time is associated with the following factors: 
a higher urgency of the driving situation, the driver not performing a non-driving related task (NDRT) such as using a handheld device, the driver receiving an auditory or vibrotactile TOR rather than no TOR or a visual-only TOR. 
Recent studies by Mok et al.~\cite{mok2017tunneled} and Eriksson et al.~\cite{eriksson2017takeover} both confirmed that drivers occupied by NDRTs have higher responses to TORs. Similarly,~\cite{feldhutter2017duration} found a significant increase in reaction time induced by NDRTs. It is further concluded that the visual distraction causes higher reaction time when it is loaded with cognitive tasks~\cite{tang2020olfactory}. Studies have also revealed several driving environments, TOR modalities
~\cite{van2017priming, tang2020olfactory}, driving expectancy~\cite{ruscio2015does}, age~\cite{walch2017car} and gender~\cite{warshawsky2002effects} associated with takeover time. The present study extend previous findings by considering various NDRTs, gender, and objective and subjective measurements of mental workload into the DeepTake framework. \par


\textbf{Takeover quality.}
In addition to takeover time, it is essential to assess the \emph{takeover quality}, which is defined as the quality of driver intervention after resuming manual control~\cite{iso21959}. 
There are a variety of takeover quality measures, depending on different takeover situations (e.g., collision avoidance, lane-keeping), including objective measures (e.g., mean lateral position deviation, steering wheel angle deviation, metrics of distance to other vehicles or objects, minimum time to collision, frequency of emergency braking) and subjective measures (e.g., expert-based assessment, self-reported experience).
Prior work has found that takeover quality can be influenced by factors such as drivers' cognitive load~\cite{du2020evaluating, zeeb2016take}, emotions and trust~\cite{dillen2020keep,du2020examining,hergeth2017prior}, and distraction of secondary NDRTs~\cite{martelaro2019exploration,dogan2019effects}. Takeover time to an obstacle\cite{zeeb2016take} has been used widely studies as an indicator of takeover performance~\cite{eriksson2017takeover}. However, a study by Louw et al.~\cite{louw2017coming} showed that takeover time and quality appear to be independent. This lack of consensus could be due to the fact that studies apply various time budget for takeover control.


\textbf{Takeover prediction.}
While existing literature mostly focus on the empirical analysis of drivers' takeover time and quality, there are a few recent efforts on the predication of drivers' takeover behavior using machine learning~(ML) approaches. 
Lotz and Weissenberger~\cite{lotz2018predicting} applied a linear support vector machine (SVM) method to classify takeover time with four classes, using driver data collected with a remote eye-tracker and body posture camera; the results achieve an accuracy of 61\%.
Braunagel et al.~\cite{braunagel2017ready} developed an automated system that can classify the driver's takeover readiness into two levels of low and high (labeled by objective driving parameters related to the takeover quality); their best results reached an overall accuracy of 79\% based on a linear SVM classifier, using features including the traffic situation complexity, the driver's gazes on the road and NDRT involvement.
Deo and Trivedi~\cite{deo2019looking} proposed a Long Short Term Memory (LSTM) model for continuous estimation of the driver's takeover readiness index (defined by subjective ratings of human observers viewing the feed from in-vehicle vision sensors), using features representing the driver's states (e.g., gaze, hand, pose, foot activity); their best results achieve a mean absolute error (MAE) of 0.449 on a 5 point scale of the takeover readiness index. 
Du et al.~\cite{du2020predicting,du2020predictingtake} developed random forest models for classifying drivers' takeover quality into two categories of good and bad (given by subjective self-reported ratings), using drivers' physiological data and environment parameters; their best model achieves an accuracy of 70\%.

In summary, the existing works only focus on the prediction of either takeover time or takeover quality. 
By contrast, DeepTake provides a unified framework for the prediction of all three aspects of takeover behavior: intention, time and quality together. 
Furthermore, DeepTake achieves better accuracy results: 96\% for takeover intention (binary classification), 93\% for takeover time (three classes), and 83\% for takeover quality (three classes).



==> DeepTakeArxiv/Sections/3-approach.tex <==
In this section, we present a novel deep neural network (DNN)-based approach, DeepTake, for the prediction of a driver's takeover behavior (i.e., intention, time, quality). Figure~\ref{fig:llustrative} illustrates an overvi-ew of DeepTake.
First, we collect multimodal data such as driver biometrics, pre-driving survey, types of engagement in non-driving related tasks~(NDRTs), and vehicle data. The multitude of sensing modalities and data streams offers various and complementary means to collect data that will help to obtain a more accurate and robust prediction of drivers' takeover behavior. 
Second, the collected multimodal data are preprocessed followed by segmentation and feature extraction. The extracted features are then labeled based on the belonging takeover behavior class. In our framework, we define each aspect of takeover behavior as a classification problem~(i.e., takeover intention as a binary classes whereas takeover time and quality as three multi-classes).
Finally, we build DNN-based predictive models for each aspect of takeover behavior. 
DeepTake takeover predictions can potentially enable the vehicle autonomy to adjust the timely initiation of TORs to match drivers' needs and ultimately improve safety. We describe the details of each step as follows. 



\subsection{Multimodal Data Sources}\label{sec:data}

\subsubsection{Driver Biometrics}
The prevalence of wearable devices has made it easy to collect various biometrics for measuring drivers' cognitive and physiological states. 
Specifically, we consider the following three types of driver biometrics in DeepTake. \par

\textbf{Eye movement.}
Drivers are likely to engage in non-driving tasks when the vehicle is in the automated driving mode~\cite{borojeni2018reading,wintersberger2018let,pakdamanian2020toward}. 
Therefore, it is important to assess the drivers' visual attention and takeover readiness before the initiation of TORs. 
There is a proven high correlation between a driver's visual attention and eye movement~\cite{zeeb2015determines,wu2019assessing,alsaid2019moving}. DeepTake uses eye movement data (e.g., gaze position, fixation duration on areas of interest) measured by eye-tracker devices. We utilize a pair of eye-tracking glasses in our user study (see Section~\ref{sec:study}).
But the aforementioned eye movement data can be captured with any eye-tracking device. \par

\textbf{Heart rate.}
Studies have found that \emph{heart rate variability} (HRV), fluctuation of heart rate in the time intervals between the nearby beats, is a key factor associated with drivers' workload~\cite{paxion2014mental}, stre-ss~\cite{dillen2020keep}, and drowsiness~\cite{vicente2011detection}.
DeepTake uses features extracted from HRV analysis for monitoring drivers' situational awareness and readiness to respond to TORs. 
Heart rate can be measured in many different ways, such as checking the pulse or monitoring physiological signals. DeepTake employes photoplethysmographic~(PPG) signal, which can be collected continuously via PPG sensors commonly embedded in smartwatches. PPG sensors monitor heart rate by the emission of infrared light into the body and measure the reflection back to estimate the blood flow.
Unlike some heart rate monitoring devices that rely on the placement of metal electrodes on the chest, PPG sensors provide accurate heart rate measures without requiring intrusive body contact. Therefore, a PPG signal is preferred for monitoring drivers' heart rate. \par

\textbf{Galvanic skin response (GSR).}
Along with HRV, GSR has been identified as another significant indicator of drivers' stress and workload~\cite{dillen2020keep,foy2018mental,mehler2012sensitivity,radlmayr2014traffic}.
A GSR signal measures the skin conduction ability. 
Drivers' emotional arousal (e.g., stress) can trigger sweating on the hand, which can be detected through distinctive GSR patterns. 
DeepTake incorporates features extracted from the GSR signal for monitoring drivers' stress levels. 
GSR sensors are also embedded in many wearable devices, including smartwatches. 


\subsubsection{Pre-Driving Survey}
In addition to the objective measurements of driver biometrics, DeepTake exploits subjective pre-driving survey responses, because drivers' prior experience and background may influence their takeover behavior~\cite{zhang2019determinants}. However, any subjective rating of factors affecting a driver's cognitive and physical ability as well as driving experience prepare a complete specification of objective metrics, potentially enhancing the distinctive attributes of an algorithm.   
DeepTake framework exerts demographic information, NASA-Task Load Index~(NASA-TLX)~\cite{hart1988development}, and the 10‐item Perceived Stress Scale~(PSS‐10)~\cite{cohen1983global} to measure drivers' perceived workload and psychological stress.
In our user study (see Section~\ref{sec:study}), we asked participants to fill in questionnaires at the beginning of each trial.

\subsubsection{Non-Driving Related Tasks (NDRTs)}
As described in Section~\ref{sec:related}, prior studies have found that engaging in NDRTs can undermine drivers' takeover performance. 
Diverse NDRTs require different levels of visual, cognitive and physical demands; thus, the influence varies when drivers are asked to interrupt the secondary task and resume manual control of the vehicle. 
DeepTake accounts for the impact of different NDRTs on the prediction of drivers' takeover behavior. 
In our user study, we considered four NDRTs in which drivers are very likely to engage in automated vehicles: (1) \textit{having a conversation with passengers}, (2) \textit{using a cellphone}, (3) \textit{reading}, and (4) \textit{solving problems} such as simple arithmetic questions~(more details in Section~\ref{sec:experimental design}). 
We chose these NDRTs because they are commonly used in driving studies~\cite{gerber2020self,dogan2019effects}, and they follow the framework of difficulty levels in the flow theory~\cite{csikszentmihalyi1990flow}. 
We further designed reading and arithmetic problem solving with two difficulty levels~(easy and medium adapted from~\cite{nourbakhsh2012using}, which reported a strong correlation between the questions and the physiological responses). 
Nevertheless, DeepTake framework can be easily adjusted to any NDRTs. 


\subsubsection{Vehicle Data}
DeepTake also considers a wide range of data streams captured from the automated vehicles, including lane position, distance to hazards, angles of the steering wheel, throttle and brake pedal angles, and the vehicle velocity. Such vehicle data can help to determine the driving condition, the urgency of a takeover situation, and the impact of drivers' takeover behavior. 


\subsection{Data Preparation}

\subsubsection{Feature Extraction and Multimodal Data Fusion}\label{sec:extraction}
The goal of DeepTake is to provide a procedure to reliably predict drivers' takeover behavior~(i.e., intention, time and quality) before a TOR initiation. Hence, the taken procedure for data preparation depends on the driving setting, collected data and the context. Herein, we incorporate data of drivers' objective and subjective measurements, as well as vehicle dynamic data. We initially apply data preprocessing techniques including outliers elimination, missing value imputation using mean substitutions, and smoothing to reduce artifacts presented in raw data. It is worth mentioning that we exclude any data stream providing insights about the unknown future~(e.g., type of alarm) or containing more than 50\% missing value. The preprocessed time series data are then segmented into 10-second fixed time windows \textit{prior to the occurrences of TORs}. In other words, if TOR happened at time t, we only used data captured in the fixed time window of [t-10s, t] and did not include any data later than t. We started with time window values of 2s and 18s, suggested in the literature~\cite{du2020predictingtake,braunagel2017ready,zhang2019determinants}, and experimentally settled on 10s, as real-world applications require a shorter time window with better prediction. We then aggregated the values of all multimodal data over this time interval, resulting in $256$ (max sampling rate)$\times 10sec=2560$ observations \textit{per takeover} event. However, depending on specific applications and contextual requirements, the selected time window length could vary. Subsequently, the segmented windows from modalities are processed to extract meaningful features describing the attributes impacting takeover behavior. 

%===============================================
%%%%%%%%%%% List of Features %%%%%%%%%%% 

% Table for Features list

\input{Tables/Features_list}


%===============================================
For the eye movement, we acquire interpolated features extracted from raw data through iMotion software~\cite{imotions}. The extracted eye movement attributes include gaze position, pupil diameters of each eye, time to first fixation, and fixation duration/sequence on the detected area of interest~(i.e., cellphone, tablet and monitor).

To compute the heart rate features, we first apply a min-max normalization on the raw PPG signal, and then filter the normalized PPG signal by applying a 2\nd order Butterworth high pass filter with a cut-off of 0.5Hz followed by a 1\st order Butterworth low pass filter with a cut-off frequency of 6Hz.
We use an open-source toolkit HeartPy~\cite{van2019heartpy} to filter the PPG signals and extract the following features from heart rate variability (HRV) analysis: the standard deviation of normal beats~(SDNN), root mean square of successive differences between normal heartbeats~(RMSSD), and the proportion of pairs of successive beats that differ by more than 50ms (pNN50). These metrics are to correlate with driver's cognitive workload and stress~\cite{peruzzini2019transdisciplinary}.


Furthermore, we obtain two common and important GSR features: the number and amplitude of peaks~\cite{manawadu2018tactical,nourbakhsh2012using}. A peak occurs when there is a quick burst of raised conductance
level. The peak amplitude measures how far above the baseline the peak occurred. Thus, peaks are valuable indicator of stress and mental workload. 


While the variety of a driver's subjective and objective measurements along with vehicle dynamic data provide complementary information to draw better insights into drivers' takeover behavior, we need to finally fuse these multimodal data into a joint representation as input to the DNN model. Beforehand, however, we employ the Z-score normalization for most of the features except extracted PPG features to accentuate key data and binding relationships within the same range. To normalize the features associated with PPG, we use the min-max normalization, as explained above. For any remaining features still containing missing values, their missing values are imputed by using their means. Table~\ref{tbl:data sources} summarizes the list of data sources and extracted features used in DeepTake. 
Finally, the generated features from each modality concatenated to create a rich vector representing driver takeover attributes. The joint representations of all feature vectors with the provision of their associated labels are eventually fed into DNN models for training. Below, the labeling procedure of these feature vectors is explained.


\subsubsection{Data Labeling}
The target labels greatly depend on the context in which the labels are presented. Herein, we define the ground truth labeling for an attribute set denoting the feature vector. Each label indicates the classification outcome of takeover intention, time, and quality that is more representative of our user study and the three takeover behavior aspects. \par

\textbf{Takeover intention.}
DeepTake classifies a driver's takeover intention into the binary outcomes, indicating whether or not the driver would resume manual control of the vehicle. In our user study, if a participant initiated the takeover action by pressing the two buttons mounted on the steering wheel~(see Figure~\ref{fig:simulator}) upon receiving a TOR, we label the feature vector as ``TK'',  showing the takeover intention; if no takeover action was initiated between the moment of TOR initiation and the incident (e.g., obstacle avoidance), we use a ``NTK'' label displaying the absence of intention. \par


\textbf{Takeover time.}
Recall from Section~\ref{sec:related} that takeover time is defined as the time period between a TOR and the exact moment of a driver resuming manual control. Prior works have considered the starting time of manual control as the first contact with the steering wheel/pedals~\cite{zeeb2015determines} or the takeover buttons~\cite{kim2017takeover}. 
In our user study, we timed the takeover moment once a participant pressed the two takeover buttons on the steering wheel simultaneously~(see Figure~\ref{fig:simulator}).
We categorize takeover time into three classes, using threshold values consistent with the pre-defined i\textsuperscript{th} percentile of takeover time in prior driving studies~\cite{coley2009driver}.
Let $T$ denote the takeover time, thus the labels are defined as  
``low'' when $T<2.6s$, ``medium'' when $2.6s\leq T\leq6.1s$, or ``high'' when $T>6.1s$. \par


\textbf{Takeover quality.}
As we alluded to earlier in Section~\ref{sec:related}, there are a wide range of metrics~\cite{iso21959} for measuring takeover quality, depending on the needs of various takeover scenarios. 
In our user study~(see Section~\ref{sec:study}), we consider a motivating scenario where the driver needs to take over control of the vehicle and swerve away from an obstacle blocking the same lane; meanwhile, the vehicle should not deviate too much from the current lane, risking crashing into nearby traffic.
Therefore, we measure the takeover quality using the lateral deviation from the current lane, denoted by $P$. In our study, we design a 4-lane rural highway with a lane width of $3.5m$. Therefore, we label the feature vectors into three classes of takeover quality:
``low'' or staying in a lane when $P<3.5m$, ``medium'' or maneuver the obstacle but too much deviations when $7m < P\leq 10m$, or ``high'' or maneuver safely and one lane deviates when $3.5\leq P\leq7m$. 




\subsection{DNN Models for Takeover Behavior Prediction}\label{sec:DNN_Model}
DeepTake utilizes a feed-forward deep neural network (DNN) with a mini-batch stochastic gradient descent.
The DNN model architecture begins with an input layer to match the input features, and each layer receives the input values from the prior layer and outputs to the next one. 
There are three hidden layers with 23, 14, and 8 ReLu units, respectively. 
The output layer can be customized for the multi-class classification of takeover intention, takeover time and takeover quality. 
For example, for the classification of takeover quality, the output layer consists of three Softmax units representing three classes~(low-, medium-, and high-) of takeover quality. 
DeepTake framework uses Softmax cross-entropy loss with an Adam optimizer with a learning rate of 0.001 to update the parameters and train the DNN models over 400 epochs. In each iteration, DeepTake randomly samples a batch of data in order to compute the gradients with a batch size of 30. Once the gradients are computed, the initiated parameters get updated. The early stopping method set to 400 epochs prevents overfitting. In addition, DeepTakes randomly divides the given labeled data into 70\% for training~(necessary for learning the weights for each node), 15\% for validation~(required to stop learning and overtraining), and 15\% for testing~(the final phase for evaluating the proposed model’s robustness to work on unseen data). Finally, in order to address imbalanced data issues where the number of observations per class is not equally distributed, DeepTake utilizes Synthetic Minority Oversampling Technique~(SMOTE)~\cite{chawla2002smote} which uses the nearest neighbor's algorithm to generate new and synthetic data.

In summary, our DeepTake framework employs different DNN models to predict takeover intention, takeover time and takeover quality. All of the DNN models in DeepTake have the same number of inputs and hidden layers, yet different output layers and associated weights. 



==> DeepTakeArxiv/Sections/4-user-study.tex <==
To test the feasibility of our proposed DeepTake framework, we conducted a user study with 20 participants featuring takeover behavior using a driving simulator\footnote{This study complies with the American Psychological Association Code of Ethics and was approved by the Institutional Review Board at University of Virginia.}. 
The following section describes the experimental setup and design of our user study as follows. 



%======================================================
\subsection{Participants}
In this study, 20 subjects~(11~female,~9~male) aged 18-30~(mean= 23.5, SD= 3.1) were recruited. All participants were hired through the university and were required to have normal or corrected-to-normal vision, to not be susceptible to simulator sickness, and to have at least one year of driving experience to be eligible for participation in this study. Before the experiment, participants were questioned as to their age and driving experience. None of them had prior experience of interaction with AVs. They were reminded of their right to abort their trial at any point with no question asked. Three participants' data were later excluded from the analysis, due to biometric data loss and a large amount of missing values. Participants received~\$20 to compensate for the time they spent in this study.



%Applying a single source of information does not seem to be an efficient way to precisely predict the takeover behavior of drivers. In this study, we used several sources of information including objective driver biometrics (eye movement, heart rate PPG signal, galvanic skin response~(GSR)), subjective measurements~(pre-driving survey), and vehicle data (see Table\ref{tbl:data sources}). All of the selected features have been previously reported in the literature to either affect or get affected by driver's cognitive and physical impairments, situation awareness, and finally readiness to takeover.



%===============================================
\begin{figure}[t!]
\centering
  \includegraphics[width=0.47\textwidth]{Figures/Study_Setup.png}
  \caption{User study setup. This custom driving simulator consists of a 30-inch monitor, a Logitech G29 steering wheel, and 10.5-inch Apple iPad Air on which the non-driving tasks are displayed. For switching between the automated and manual control of the vehicle, the participant needs to press the two blue buttons on the steering wheel simultaneously. The participant wears a pair of eye-tracking glasses, and a wearable device with GSR and PPG sensors for the biometrics acquisition.}
  \label{fig:simulator}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%===========================
\subsection{Apparatus}
Figure~\ref{fig:simulator} shows our low fidelity driving simulator setup, which consists of a Logitech G29 steering wheel, accelerator, brake pedal and paddle shifters. The simulator records driver control actions and vehicle states with a sampling frequency of 20Hz and sent the captured data through a custom API using iMotions software~\cite{imotions}. The simulated driving environments along with the tasks were created using PreScan Simulation Platform. The driving environment was displayed on a 30-inch monitor. The distance between the center of the Logitech G29 steering wheel and the monitor was set at 91cm. A set of stereo speakers was used to generate the driving environment sounds along with the auditory alarm of TORs~(more details in Section~\ref{sec:experimental design}). An Apple iPad Air (10.5-inch) was positioned to the right side of the driver and steering wheel to mimic the infotainment system and displayed an article for NDRT. 

We used Tobii Pro-Glasses 2 with the sample rate of 60Hz to collect the eye movement data, and a Shimmer3+ wearable device with a sampling rate of 256Hz to measure PPG and GSR signals. To maintain consistency across all participants, we positioned the Shimmer3+ to the left of all subjects. This consistency helps reduce the motion artifact where the subjects needed to frequently interact with the tablet on the right-hand side. Although we designed our scenarios in a way to minimize the inevitable motion artifacts, we performed necessary signal processing on the PPG and GSR signals to remove potentially corrupted data, as discussed in Section~\ref{sec:data}.

% %===============================================
% % Table for modalities
% \vspace{-1mm}
% \input{Tables/TOR_Modalities}
% \vspace{-1mm}
% %===============================================


% \begin{figure*}
% \centering
% %% left-hand side: a single subfigure
%     \begin{subfigure}{0.5\textwidth}
%         \includegraphics[width=4.83in,height=208pt]{Figures/Map_2Colors.png}
%         \centering
%         \caption{Map of simulated drive} \label{subfig:left}
%     \end{subfigure}
%         %% horizontal separation between the left and right hand sides
%     \hspace*{\fill}
%         %% right-hand side: a minipage that contains two more subfigures
%     \begin{minipage}{0.3\textwidth}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth,height=103pt]{Figures/Driving_Scene2.png}
%         %\caption{Takeover situation scenario} \label{subfig:upper-right}
%     \end{subfigure}
%         %\vspace*{0.5cm}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth,height=103pt]{Figures/Driving_Scene.png}
%         \caption{Takeover situation scenarios} \label{subfig:lower-right}
%     \end{subfigure}
%     \end{minipage}
% \caption{ a) Shows the selected route for the round-trip driving task. All 15 TOR warnings with a 60-90sec time interval between them are shown; b) Displays the takeover scenarios where a disabled vehicle (top figure)/working zone (bottom figure) block the road ahead. In each scenario, drivers have up to 10sec to react properly. In both cases the system is still on Auto mode and will change to manual as soon as the driver initiates the takeover.}
% \end{figure*}

%===============================================
%\subsection{Questionnaires}
% Reaction time depends on so many factors which are not directly accessible and must be evaluated. Therefore, in this study we combined subjective and objective assessments. The following subjective measurements accompanied by responses from wearable devices helped us to obtain the level of stress and workload, the so-called ground truth that we might have overlooked by relying on physiological data alone.



\subsection{Experimental design} \label{sec:experimental design}
A within-subjects design with independent variables of stress and cognitive load manipulated by NDRTs and the TOR types was conducted with three trials in a controlled environment as shown in Figure~\ref{fig:simulator}. We designed driving scenarios in which the simulated vehicle has enough functionality similar to AVs, such that the full attention of the driver was not required at all times. \par

\textbf{Non-Driving Related Tasks.} We used four common NDRTs with various difficulty levels and cognitive demand as shown in Table~\ref{tbl:SecondaryTasks}. Participants used the tablet to read the designated articles and answer the arithmetic questions. Additionally, they were asked to use their own hand-held phones, needed for the browsing tasks. Each participant performed all NDRTs with the frequency of four times in each trial~(except for solving the arithmetic questions which occurred three times;$15\times3$ in total). The conditions and the three driving scenarios were counterbalanced among all participants to reduce order and learning effects. To have natural behavior to the greatest extent possible, participants were allowed to depart from NDRTs to resume control of the vehicle at any given time. During manual driving, participants controlled all aspects of the vehicle, including lateral and longitudinal velocity control. 
%===============================================
\input{Tables/NDRTs.tex}
%===============================================


%===============================================
%%%%%%
\begin{figure*}[t!]
   \centering
   \includegraphics[width=6.5in]{Figures/Fig2-scenario.pdf}
   \caption{ A schematic view of an example of a takeover situation used in our study, consisting of: 1) takeover timeline associated with participants’ course of action; 2) system status; and 3) takeover situation. The vehicle was driven in the automated mode to the point after the TOR initiation and transitioning preparation period. The ego vehicle is shown in red and the lead car is white. When the Ego vehicle reaches its limits, the system may initiate~(true alarm) or fail~(no alarm) to initiate the TOR, and the driver takes the control back from the automated system.}
   \label{fig:Scenario}
\end{figure*} 
%%%%%%
%===============================================
\textbf{Driving Scenarios.} The driving scenarios comprised a 4-lane rural highway, with various trees and houses placed alongside the roadway. 
We designed five representative situations where the AVs may need to prompt a TOR to the driver, including novel and unfamiliar incidents that appear on the same lane. Figure~\ref{fig:Scenario} shows an example of a takeover situation used in our study.
The designed unplanned takeovers let participants react more naturally to what they would normally do in AVs~\cite{mccall2019taxonomy} or as introduced by Kim and Yang~\cite{kim2017takeover}, participants' reaction times are in detectable categories. In other words, participants have no previous knowledge of incident appearance, which might happen among other incidents requiring situational awareness and decision-making. 
 


\textbf{Takeover Requests.} In order to incorporate DeepTake in the design of adaptive in-vehicle alert systems in a way that not only monitors driver capability of takeover, but also to enhance takeover performance of automated driving, various types of TOR were required. An auditory alarm was used to inform participants about an upcoming hazard that required takeover from the automated system. The warning was a single auditory tone (350Hz, duration: 75ms) presented at the time of hazard detection~($\approx$140m or $\approx$13sec before the incidents, depending the speed of the vehicle). In a precarious world, AVs should be expected to fail to always provide correct TORs. Herein, the scenarios were constructed conservatively to include flawed TORs by which subjects would not over-trust the system's ability. In other words, the scenario demands that the participant be partially attentive and frequently perceive the environment. In order to cover the scenarios that one might encounter while driving an AV, we designed multiple critical types of TORs, including an explicit alarm (true alarm), silent failure (no alarm), and nuisance alarm (false alarm). True alarm indicates the situation in which the system correctly detects the hazard and triggers a TOR, no alarm represents the system's failure to identify the existing hazard, and false alarm presents misclassification of a non-hazardous situation as an on-road danger requiring takeover. We randomized the 15 TOR occurrences in each trial~(45 in total for each participant) with 6, 3, 6 repetitions for true alarm, no alarm, false alarm, respectively. 
In addition, we also designed an information panel where the participants could see the status of the vehicle along with the cause of TOR~(see Figure~\ref{fig:simulator}). 




\subsection{Procedure} \label{sec:Procedure}
Upon arrival in the lab, participants were asked to sign a consent form and fill out a short demographic and driving history questionnaires. 
Subsequently, they were briefed on how the automated system functions, how to enable the system by simultaneously pressing two blue buttons on the steering wheel, and what they would experience during NDRTs. They were further instructed that if the system detected a situation beyond its own capabilities to handle, it would ask~(true alarm) or fail to ask~(no alarm) to take over control. Afterward, participants completed a short training drive along a highway for a minimum of 5 minutes to get familiar with the driving and assure a common level of familiarity with the setup, NDRTs, and auditory signals pitch. 

Once the subjects felt comfortable with the driving tasks and NDRTs, they proceeded to the main driving scenario. Prior to beginning the main experiment, we calibrated the eye-tracking glasses~(repeated at the beginning of each trial) and set participants up with the Shimmer3+ wearable device. Then, participants were required to complete the baseline NASA-TLX questionnaire followed by the PSS-10 questionnaire. The participants were also instructed to follow the lead car, stay on the current route, and follow traffic rules as they normally do. The participants were cautioned that they were responsible for the safety of the vehicle regardless of its mode~(manual or automated). Therefore, they were required to be attentive and to safely resume control of the vehicle in case of failures and TORs. Since the scenarios were designed to have three types of TORs, they needed to adhere to the given instruction whenever they felt the necessity. The given instruction enabled the drivers to respond meticulously whenever it was required and to reinforce the idea that they were in charge of the safe operation of the vehicle.  Due to the system's limitations, participants were told to maintain the speed within the acceptable range~($<47$mph). The experiment was conducted utilizing scenarios consisting of sunny weather conditions without considering the ambient traffic. The order of NDRT engagement was balanced for participants~(see Figure~\ref{fig:Scenario}).

The remainder of the experiment consisted of three trials, each containing 15 TORs, followed by a 5-minute break between trials. At the end of each trial, participants were requested to fill out the NASA-TLX.  After completion of the last trial, participants filled out the last NASA-TLX followed by a debrief and a \$20 compensation. The experiment took about one hour for each participant.



==> DeepTakeArxiv/Sections/5-results.tex <==

We evaluate the performance of DeepTake framework using the multimodal data collected from our user study.
We describe the baseline methods, metrics, results, and analysis as follows. 

% \todo{introduce other machine learning methods, feature selection...}
\subsection{Baseline Methods}
Overall, we obtained about 2 million observations to train, test, and validate DeepTake with; 2560 observations per TOR $\times~15$ TORs per trial $\times~3$ trials $\times~17$ subjects. We evaluate the performance of DeepTake DNN-based models with six other ML-based predictive models, including Logistic Regression, Gradient Boosting, Random Forest, Bayesian Network, Adaptive Boosting~(Adaboost), and Regularized Greedy Forest~(RGF). Our process of choosing the ML models is an exploratory task with trials and tests of multiple off-the-shelf algorithms and choosing those that perform the best.
To evaluate the prediction performance of DeepTake framework with other ML models, we were obligated to utilize some feature importance techniques. The reasons to apply feature importance techniques for an ML algorithm are: to train the predictive model faster, reduce the complexity and increase the interpretability and accuracy of the model. In order to do so, after splitting the labeled data into training, testing, and validation sets~(see Section~\ref{sec:DNN_Model}), we employ the following feature importance methods on each training set: Absolute Shrinkage and Selection Operator~(LASSO), and random forest. LASSO helps us with not only selecting a stable subset of features that are nearly independent and relevant to the drivers' takeover behavior, but also with dimensionality reduction. The random forest method, on the other hand, ranks all of the features based on their importance levels with the drivers' takeover behavior. The overlapped features chosen by the two methods were used to train the ML-based classification models of takeover behavior.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Metrics}
We apply 10-fold cross-validation on training data to evaluate the performance of selected features in the prediction of driver takeover intention, time and quality. Cross-validation provides an overall performance of the classification and presents how a classifier algorithm may perform once the distribution of training data gets changed in each iteration. In cross-validation, we utilize the training fold to tune model hyper-parameters (e.g., regularization strength, learning rate, and the number of estimators), which maximizes prediction performance. Therefore, we train predictive models with the best hyper-parameters. Cross-validation randomly partitions the training data into n subsets without considering the distribution of data from a subject in each set. A possible scenario is that data from one subject could be unevenly distributed in some subsets, causing overestimation of the prediction performance of a model. To avoid this situation, we check the subjects' identifiers in both the training and testing sets to ensure that they belong to just one group. We achieve this by forcing the subject to be in one group.
To determine the \textit{accuracy} of the binary classification of takeover intention performed by predictive models, accuracy was defined as
$Acc = \frac{TP+TN}{TP+TN+FP+FN}$
(TP, TN, FP, and FN represent True Positive, True Negative, False Positive, and False Negative, respectively). 
%TP and TN correspond to correct classification and FP and FN correspond to false or incorrect classification. 
For the multi-class classification of takeover time and quality, we used the average accuracy per class.
We also used the metric of \emph{weighted F1 scores} given by 
\begin{equation}
    W F_1 = \sum_{n=1}^{l} \frac{2\times Pr_i\times Rc_i}{Pr_i+Rc_i}\times W_i,
\end{equation}
where $Pr_i = \frac{\sum_{i=1}^{l}\frac{TP_i}{TP_i+FP_i}}{l}$ is the precision, 
$Rc_i = \frac{\sum_{i=1}^{l}\frac{TP_i}{TP_i+FN_i}}{l}$ is the recall, and 
$W_i$ is the weight of the $i^{th}$ class depending on the number of positive examples in that class. It is worth mentioning that to deal with our imbalanced data, where the number of observations per class is not equally distributed, DeepTake framework along with ML-based predictive models use SMOTE to have a well-balanced distribution within class~(see Section~\ref{sec:DNN_Model}).


Given multiple classifiers, we use the \textit{Receiver Operating Characteristic}~(ROC) curve to compare the performance of DeepTake alongside other ML-based models. 
The ROC curve is a widely-accepted method that mainly shows the trade-off between TP and FP rates. A steep slope at the beginning of the curve shows a higher true positive~(correct) classification of the algorithm, whereas increasing the FP rate causes the curve to flatten. The ROC curve provides an effective way to summarize the overall performance of classification algorithms by its only metric, AUC. The AUC values provided in Figure~\ref{fig:ROC} can be interpreted as the probability of correctly classifying the driver takeover behavior into the candidate category compared to a random selection~(black line in Figure~\ref{fig:ROC}).

In addition, we use the \textit{confusion matrix} to further illustrate the summary of DeepTake's performance on the distinction of takeover intention, time, and quality per class.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Results and Analysis}

Multiple classification algorithms were employed to compare the performance of DeepTake on obtaining a reliable discriminator of driving takeover behavior, including intention, time, and quality. As the prediction of driver takeover time and quality are contingent upon the driver's intention to take over from the autonomous systems after receiving TOR, the classification algorithms were initially carried out on this first stage of driver takeover prediction, followed by takeover time and quality. 

%%%%%%%%%%% Table for model comparison %%%%%%%%%%%%%
\vspace{1mm}
\input{Tables/Model_Comparision}
\vspace{0.1mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%% Accuracy Vs Loss %%%%%%%%%%% 
\begin{figure*}[t!]
\centering
   \includegraphics[width=\textwidth]{Figures/ROC_ALL_test_4.png}
   \caption{The ROC curve comparison of our DeepTake and six ML classification algorithms for classification of takeover behavior: (a) takeover intention, (b) takeover time, and (c) takeover quality. The ROC curve shows the average performance of each classifier and the shadowed areas represent the 95\% confidence interval. The macro AUC associated with each classifier is shown where AUC value of 0.5 refers to a chance.[Best viewed in color]}
   \label{fig:ROC}
\end{figure*} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\textbf{Takeover intention.}
Analysis of the binary classification of drivers' takeover intention is shown in Table~\ref{tbl:results comparison}. The results show that DeepTake outperforms other ML-based models. However, among the ML-based algorithms, RGF attains the highest accuracy and weighted F1 score~(92\% and 89\%) followed by AdaBoost~(88\% and 88\%) and Logistic Regression~(77\% and 88\%). Moreover, ROC was applied in order to better evaluate each of the classifiers. Figure~\ref{fig:ROC}.a shows ROC curves and AUC values for all six ML models along with DeepTake to infer the binary classification of takeover intention. Although DeepTake shows outperformance on correctly classifying a driver's intention~(AUC=0.96) using the multimodal features, RGF shows promising performance with an AUC of 0.94. Similar to the accuracy level, AdaBoost had a slightly lower performance with an AUC= 0.91. Furthermore, we obtained the confusion matrix for takeover intention~(Figure ~\ref{fig:CM-All}.a) showing that the percentage of misclassifications is insignificant. Table~\ref{tbl:results comparison}, together with the results obtained from the AUC in Figure~\ref{fig:ROC}.a and the confusion matrix in Figure ~\ref{fig:CM-All}.a, ensure that our multimodal features with the right DNN classifier surpass the takeover intention prediction. 

\vspace{-1mm}
%%%%%%%%%%% Accuracy Vs Loss %%%%%%%%%%% 
\begin{figure}[b!]
\centering
   \includegraphics[width=0.5\textwidth]{Figures/AccuracyVSLoss.pdf}
    % \vspace{3mm}
   \caption{The top graph shows the prediction accuracy of training and test sets for 400 epochs, whereas the bottom graph indicates the loss for  DeepTake on prediction of three classes of low-, mid-, and high- takeover time.}
   \label{fig:Model_Accuracy_vs_Loss}
\end{figure} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%% Confusion Matrix 3_Class %%%%%%%%%%% 
\begin{figure*}[t!]
\centering
  \includegraphics[width=\textwidth]{Figures/CM_ALL.png}
  \caption{Confusion matrix for the prediction of takeover behavior.The results are averaged over 10 fold cross validation splits. (a) Binary class takeover intention takeover(TK) vs. Not Takeover(NTK), (b) 3-Class classification results of takeover time, (c) 3-class classification of takeover quality.}
  \label{fig:CM-All}
\end{figure*}
%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 

\textbf{Takeover time.}
DeepTake's promising performance in takeover intention estimation leads us to a more challenging multi-class prediction of driver takeover time. As some of the ML-based models attained reasonably high accuracy in the binary classification of takeover, their performances, along with our DeepTake DNN based in classifying multi-class classification of takeover time could assess the robustness of the DeepTake.






Figure\ref{fig:ROC}.b shows a comparison amongst the models explored in this paper along with DeepTake for prediction of takeover time. It displays that DeepTake produces the best overall result with an AUC value of 0.96 $\pm$ 0.02 for each takeover low-, mid-, and high- time.
We next consider the accuracy comparison of our DeepTake model with other classifier algorithms, reported in Table~\ref{tbl:results comparison}. It is evident that DeepTake outperforms all of the classic algorithms. In the three-class classification of takeover time~(low,~mid,~high), DeepTake achieves a weighted-F1 score of 0.87, thereby achieving the best performance on this task by a substantially better accuracy result of 92.8\%. Among the classifiers, RGF and AdaBoost still performed better~(73.4\% and 64.1\%). As shown in Figure~\ref{fig:Model_Accuracy_vs_Loss}, DeepTake gained a high accuracy for both the training and testing sets. However, the model did not significantly improve and stayed at around 92\% accuracy after the epoch 250. 








% \begin{figure}[h!]
%      \centering
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/CM-TK.png}
%          \caption{}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/cm_threeclass_noNum-2.png}
%          \caption{}
%      \end{subfigure}
%     \hfill
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/CM-3CL-Quality.png}
%          \caption{}
%      \end{subfigure}
% \caption{Steering behavior after receiving TORs.}\label{fig:Trajectory_time}     
% \end{figure}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To capture a better view of the performance of DeepTake on the prediction of each class of takeover time, we also computed the confusion matrix. Figure~\ref{fig:CM-All} displays the performance of DeepTake DNN model as the best classifier of three-class takeover time. As the diagonal values represent the percentage of elements for which the predicted label is equal to the true label, it can be seen that the misclassification in medium takeover time is the highest. Also, marginal misclassifications are found in the 2\%-5\% of the high and low takeover time classes, respectively. Overall, all three evaluation metrics of AUC, accuracy, and confusion matrix indicate that DeepTake robustness and promising performances in correctly classifying the three-class takeover time.




\textbf{Takeover quality.}
The test accuracy results of the 3-class classification of all classifiers are presented in Table~\ref{tbl:results comparison}. DeepTake achieves the highest accuracy with an average takeover quality of 83.4\%. While the value of RGF was close to DeepTake, the rest of the algorithms were not reliable enough to discriminate each class of takeover. However, we should note that RGF training time is very slow and it takes about two times longer than DeepTake to perform prediction.

In addition, Figure~\ref{fig:ROC}.c presents the multi-class classification of takeover quality. Analysis of the discriminatory properties of DeepTake achieve the highest AUC of 0.92 $\pm$ 0.01 scores among the other models for each individual class. RGF model yields an impressive average macro AUC of 0.91. Such a model indicates a high-performance achievement with informative features.

We further investigated DeepTake robustness in correctly classifying each class of takeover quality and the results achieved by the method are shown in Figure~\ref{fig:CM-All}.c. For the 3-class quality estimation, DeepTake achieved an average accuracy of 87.2\%.








% %%%%%%%%%%% Car trajectory %%%%%%%%%%% 
% \begin{figure}[t!]
% \centering
%   \includegraphics[width=0.6\textwidth]{Figures/Trajectory_V3.png}
%   \caption{Lateral position of the vehicle.}
%   \label{fig:Trajectory}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Figure \ref{fig:Trajectory}  shows the mean lateral position of the vehicle in the cases that the drivers took over. The shadow represents 95\% confidence interval. The center-front of the vehicle is used as the reference point. Time "0" marks the time when the vehicle passed the obstacle. In other words, Figure \ref{fig:Trajectory} depicts the lateral trajectory from 10 second before passing the obstacle to 10 second after. It demonstrates that the takeover quality is impacted by the type of alarms. Under the impact of the true alarm, the vehicle deviates less than when there is no alarm. In addition, the drivers reacted earlier for the true alarm. To be noted, we also found there are few cases (15 cases) that the drivers accidentally took over for the false alarm. Similarly, Figure \ref{fig:Trajectory_2} shows the lateral position with respect to different takeover time. It can be seen that the higher the takeover time is, the farther the vehicle deviates when passing the obstacle.

% %%%%%%%%%%% Car trajectory %%%%%%%%%%% 
% \begin{figure}[t!]
% \centering
%   \includegraphics[width=0.6\textwidth]{Figures/TrajectorywstTime.png}
%   \caption{Lateral position of the vehicle.}
%   \label{fig:Trajectory_2}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> DeepTakeArxiv/Sections/6-discussion.tex <==


\subsection{Summary of major findings}
In the current design of takeover requests, AVs do not account for human cognitive and physical variability, as well as their possibly frequent state changes. In addition, most previous studies emphasize the high-level relationships between certain factors and their impacts on takeover time or quality. However, a safe takeover behavior consists of a driver's willingness and readiness together. The focus of this paper is to utilize multimodal data into a robust framework to reliably predict the three main aspects of drivers' takeover behavior: takeover intention, time and quality. To the best of our knowledge, the DeepTake framework is the first method for the estimation of all three components of safe takeover behavior together within the context of AVs and it has also achieved the highest accuracy compared to previous studies predicting each aspect individually. To ensure the reliability of DeepTake's performance, we applied multiple evaluation metrics and compared the results with six well-known classifiers. Despite the promising accuracy of some of the classifiers, namely the RGF classifier, the accuracy of DeepTake surpassed in its prediction of takeover behavior. In general, our model performed better in classifying driver takeover intention, time and quality with an average accuracy of 96\%, 93\%, and 83\%, respectively.

%%%%%%%%%%% Confusion Matrix 5_Class %%%%%%%%%%% 
\begin{figure}[t!]
\centering
  \includegraphics[width=0.48\textwidth]{Figures/CM_FiveCL_RT.png}
  \caption{Confusion matrix for the prediction of five classes of driver takeover time.}
  \label{fig:CM-FiveClass}
\end{figure}
%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 

% % %%%%%%%%%%% Car trajectory %%%%%%%%%%% 
\begin{figure*}[t!]
\centering
  \includegraphics[width=7.5in]{Figures/fig_trajectory/Trajectory4final_2.pdf}
  \vspace{1mm}
  \caption{Average trajectories when drivers took over control from automated system after receiving TORs. Top graph shows the lateral position of the vehicle with respect to no alarm~(silent failure) and true alarm~(explicit alarm). Bottom graph shows the lateral position of the vehicle for three categories of takeover time (low, mid, and high). The light shaded area representing standard deviation at each time point.}
  \label{fig:Trajectory_time} 
\end{figure*}
% % %%%%%%%%%%% Car trajectory %%%%%%%%%%% 

In order to further assess the robustness of DeepTake, we increase the number of classes to the more challenging five-class classification of takeover time where the classes defined as ``lowest'' when $T<1.5s$, ``low'' when $1.5s\leq T<2.6s$, ``medium'' when $2.6s\leq T<4.7s$, ``high'' when $4.7s\leq T\leq6.1s$, or ``highest'' when $T>6.1s$. Figure~\ref{fig:CM-FiveClass} represents the performance of DeepTake on classifying the five-class takeover time. Although DeepTake was not as distinctive in five-class classification as in the three-class, it still achieved promising results. Lowest, high, and medium takeover times are the top three pairs that were the most frequently misclassified by the  DNN model. The reason might be that the selected features do not have the required distinctive characteristics to perfectly divide the low and medium takeover time. In each class, it could still distinguish between five other classes with an average accuracy of 77\%. With a future larger amount of data collection satisfying each class need,  DeepTake could further improve its distinctive aspect of each feature for more precise classification. 


\subsection{Descriptive analysis of takeover time and quality}
Although DeepTake takes advantage of a DNN-based model integrated into its framework, understanding the reasons behind its predictions is still a black-box and a challenging problem which will be tackled in our future works. However, to comprehend the effects of multimodal variables on takeover time and quality, a repeated measure Generalized Linear Mixed~(GLM) model with a significance level of $\alpha$ = 0.05 to assess the correlation of suboptimal features was used to predict takeover time and quality. The analysis of the results shows the significant main effect of NDRTs on takeover time and quality~($F_{3,28}=13.58$, $p<0.001$) followed by fixation sequence~($F_{1,28}=35.87$, $p<0.001$) and vehicle velocity~($F_{1,28}=13.06$, $p<0.001$). Post-hoc tests using Bonferroni demonstrated a higher impact of interaction with the tablet and reading articles~($p<0.001$) as opposed to a conversation with passengers. This result could be based on the amount of time spent and the level of cognitive load on the takeover task. This finding is aligned with the previous results of~\cite{feldhutter2017duration,eriksson2017takeover}. Additionally, there was no significant effect of brake and throttle pedal angle on the takeover time($F_{1,28}=3.05$, $p=0.085$) and quality~($F_{1,28}=1.27$ $p=0.256$). This could be because our scenarios did not take place on crowded roads and participants were not forced to adopt a specific behavior after the TOR. Therefore, they could maneuver the vehicle without significant adjustment to either pedal.



%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
% % \vspace{-5mm}
% \begin{figure*}[t!]
% \vspace{1mm}
%      \centering
%      \begin{subfigure}[t]{0.47\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/first_traj_edit.png}
%          \caption{The lateral position of the vehicle with respect to silent failure~(No-Alarm) and explicit alarm~(True Alarm).}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.47\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/second_traj_edit.png}
%          \caption{Examining the relationship between lane position and the class of takeover time.}
%      \end{subfigure}
%      \vspace{3mm}
% \caption{Average trajectories when drivers took over control from automated system after receiving TORs.}\label{fig:Trajectory_time}     
% \end{figure*}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



On the other hand, takeover quality tied into drivers' lane keeping control and was impacted by the alarm type and the category of takeover time shown in Figure~\ref{fig:Trajectory_time}. Although we did not consider the type of alarm and category of takeover time for prediction of takeover behavior as they could simply manipulate DeepTake outcomes by providing insights about the future, it is worth additional investigation of their impacts on the takeover quality. Since participants' takeover times and the speed of the vehicle on the manual driving were different, Figure~~\ref{fig:Trajectory_time} shows the average time of TOR. The top graph in Figure~\ref{fig:Trajectory_time} depicts the average lateral position of the vehicle with respect to no alarm and true alarm. These two types of the alarm were considered due to the necessity of taking over. Under the impact of the true alarm, the vehicle deviates less than when there is no alarm, yet not significantly~($F_{2,28}=7.07$, $p=0.78$). Moreover, the drivers performed more abrupt steering wheel maneuvers to change lanes on true alarm. Similarly, the bottom graph in Figure \ref{fig:Trajectory_time} shows the lateral position with respect to different takeover times~(low, mid, and high). It can be seen that the longer the takeover time is, the farther the vehicle deviates from the departure lane. Differences in takeover time were also analyzed to investigate the takeover quality. The main effect of the type of takeover time was not significant~($F_{2,19}=0.44$). Although prior research has revealed various timing efforts to fully stabilize the vehicle~\cite{merat2014transition}, our observations are comparable to~\cite{naujoks2019noncritical} and \cite{bueno2016different}.




\subsection{Implications on the design of future interactive systems}

We believe that our human-centered framework makes a step towards enabling a longer interaction with NDRTs for automated driving. DeepTake helps the system to constantly monitor and predict the driver's mental and physical status by which the automated system can make optimal decisions and improve the safety and user experience in AVs. Specifically, by integrating the DeepTake framework into the monitoring systems of AVs, the automated system infers when the driver has the intention to takeover through multiple sensor streams. Once the system confirms a strong possibility of takeover intention, it can adapt its driving behavior to match the driver's needs for acceptable and safe takeover time and quality. Therefore, a receiver of TOR can be ascertained as having the capability to take over properly, otherwise, the system would have allowed the continued engagement in NDRT or warned about it. Thus, integration of DeepTake into the future design of AVs facilitates the human and system interaction to be more natural, efficient and safe. Since DeepTake should be used in safety-critical applications, we further validated it to ensure that it meets important safety requirements~\cite{grese2021formal}. We analyzed DeepTake sensitivity and robustness with several techniques using the Marabou verification tool. The sensitivity analysis provides insight into the importance of input features, in addition to providing formal guarantees with respect to the regions in the input space where the DeepTake behaves as expected. \par
DeepTake framework provides a promising new direction for modeling driver takeover behavior to lessen the effect of the general and fixed design of TORs which generally considers homogeneous takeover time for all drivers. This is grounded in the design of higher user acceptance of AVs and dynamic feedback~\cite{seppelt2019keeping,ekman2017creating}. The information obtained by DeepTake can be conveyed to passengers as well as other vehicles letting their movement decisions have a higher degree of situational awareness.
We envision that DeepTake would help HCI researchers and designers to create user interfaces and systems for AVs that adapt to the drivers’ state.



\subsection{Limitations and future work}
The following limitations should be taken into consideration for future research and development of DeepTake. \\
First, it is acknowledged that the DeepTake dataset is vulnerable to the low fidelity driving simulator used for data collection. It is possible that the takeover behavior of subjects were influenced by the simplicity of driving setup and activities. To apply DeepTake on the road, we will need more emphasis on various user's activities and safety, and exclude subjective surveys causing biases. Second, while we increased the number of classes, future development of DeepTake should predict takeover time numerically. For this purpose, a larger dataset will be needed which accounts for a high variation of individual takeover time and probabilistic nature of DNNs by which the DeepTake framework can still learn and reliably predicts takeover time. 

Third, although we tried to avoid overfitting, it is possible that DeepTake emphasized more on few features that frequently appeared in TORs, and the performance may not be the same if more scenarios are being tested. Thus, DeepTake decision boundaries need to be experimented with different adversarial training techniques.  
Forth, DeepTake lacks using real-world data which often significantly different and could potentially impact the results of DeepTake framework. Testing the framework on real-world data helps users to gain confidence in DeepTake's performance. DeepTake was developed and assessed offline using a driving simulator in a controlled environment. Future work should explore the deployment of DeepTake online and in the wild for real-world applications in future AVs. We plan to integrate the DeepTake and its verification results~\cite{grese2021formal} into the safety controller, which will be then evaluated using the on-road vehicle. In our
future work we also plan to try to reduce the number of features in the model by using the results from the sensitivity analysis along with feature importance analysis techniques~(i.e. LIME and SHAP) to discover features that may be able to be dropped from the model. 

%Therefore, there is a need to inspect DeepTake performance using real-world data.


















==> DeepTakeArxiv/Sections/7-conclusion.tex <==

 

In this work, we present DeepTake, a novel method that predicts driver takeover intention, time and quality using data obtained from the vehicle, wearable sensors, and a self-administered survey taken before driving. By using DNN-based models, DeepTake enables prediction of driver takeover intention, time and quality, all of which are crucial in ensuring the safe takeover of an automated vehicle. Our evaluation showed that DeepTake outperforms the best accuracy results of prior work on takeover prediction with an accuracy of 96 \%, 93 \%, and 83\% for the multi-class classification of takeover intention, time and quality, respectively. 
As prior studies demonstrated, alarming drivers when the system detects a situation requiring takeover does not guarantee safe driver takeover behavior ~\cite{korber2018have, lee2020analysis, mcdonald2019toward}. We believe that accurate takeover prediction afforded by DeepTake would allow drivers to work on non-driving related tasks while ensuring that they safely take over the control when needed. DeepTake opens up new perspectives for HCI researchers and designers to create user interfaces and systems for AVs that adapt to the drivers’ context.

% We believe that the prediction results of DeepTake can enable HCI researchers and designers to create future interactive systems for AVs that adapt to the drivers' context, guarantee the safety, and improve the user experience.



==> DeepTakeArxiv/Sections/8-Acknowledgment.tex <==
We would like to thank Prof. Corina P\u{a}s\u{a}reanu from Carnegie Mellon University and Prof. Radu Calinescu from University of York for their valuable inputs, and John Grese for his help in evaluating DeepTake with a high number of epochs. This work was supported in part by National Science Foundation CCF-1942836 grant, Assuring Autonomy International Programme, and Toyota InfoTech Labs.



==> DeepTakeArxiv/Sections/oldSections/Introduction.tex <==

Automated vehicles~(AVs)~\cite{sae2018taxonomy}) have been introduced with the aim of rapidly improving functionality, to the degree that highly automated driving will be introduced to the general public within the next few years. Audi’s traffic jam pilot, Tesla’s Autopilot, Mercedes' Distronic Plus are only a few examples of such commercially available vehicles~\cite{boelhouwer2019turmoil,menzel2018scenarios}. AVs let drivers take their hands off the wheel and their attention away from the primary task of driving~\cite{nhtsa2013department,mccall2019taxonomy}.  However, there are still challenging scenarios for AVs to safely maneuver wherein human should backup~(e.g., country roads with poorly visible lane markings, and other unfamiliar incidents)~\cite{banks2018driver,louw2017coming}. To cope with AVs' needs for constructive collaboration with human, we present DeepTake, a deep neural network~(DNN)-based framework for robust prediction of drivers' takeover behavior using multimodal data.

Despite automated systems have seen undeniable advances in the recent years, the commonality of their human-automation interaction design has not been thoroughly adapted to the new role of the driver as a fallback ready~\cite{tenhundfeld2020trust,hancock2019future,endsley2017here}. As we may be many years away from the fully-automated vehicles which can replace conventional, human-driven vehicles, it is important that the automated system constantly estimates how receptive the human is to the hazardous situations as early as possible to the extent of being able to takeover control from the automated system in a safe manner. This will potentially alleviate the safety concerns associated with the driver's status, engaged in non-driving-related tasks (NDRTs), inattentive, and fatigued, prior to takeover the vehicle control.

Currently, the Society of Automotive Engineers~(SAE) dictates that drivers need to be available to intervene when a transition to driver is crucial based on preset requirements or limitations in the automated system~\cite{lee2018perspectives,endsley1995out}. In this transition, the automated system prompts the driver concerning the vehicle status and asks to relinquish control~(takeover request or TOR) of the vehicle to the driver~\cite{bazilinskyy2017usefulness}. This requires drivers to takeover from the automated system in a given limited time~\cite{zeeb2016take}. However, shifting the role from a passive monitor who may have engaged with NDRTs for a prolonged time to an active controller in a timely manner may in fact leave the driver in a less capable state to make life-saving decisions. 
% But, what would happen if the automated system estimates how long the driver would take to resume and safely control the vehicle~(e.g., more than the time to collide)?
% Explain the need and how we solve it
Furthermore, overloaded, tired, and distracted drivers may need more time than their normal conditions to respond properly and the system needs to facilitate it by predicting driver's status before initiating TOR. 

Transitioning to manual control introduces two challenges for proper takeover performance: (1)~\textit{when} human will be able to takeover~\cite{eriksson2017takeover,zeeb2016take}, and (2)~\textit{how} adequately safe human will regain the control~\cite{happee2017take}. The safety countermeasures or \textit{"takeover quality"} is relatively interconnected to timing of the reaction as the longer reaction time to a TOR may increase the chance of proper controlling of the vehicle~\cite{louw2017coming,gold2013take}. Nevertheless, the driver's reaction time and the relevance of takeover quality depends on the contextual environment, the vehicle's and driver's status. Therefore, robust prediction of \textit{when} and \textit{how} human performs takeover is critically challenging for safe and timely transfer of control. 




%  Therefore, there is a need for a data driven monitoring system which reliably predicts drivers reaction time and the possible quality of takeover.

% it may not request human interference until the driver is fully capable of doing so. This paper develops a novel framework for the prediction of the driver's reaction time using Deep Neural Network~(DNN). 
% To the best of our knowledge, this is the first DNN-based model which extracts features from multiple wearable sensors along with vehicle trajectory information to perform reaction time classification. 


To address the above challenges, we present a framework utilizing multiple sources of information to reliably estimate three phases of driver's takeover behavior before initiating TORs. Our framework predicts driver's: (1) takeover intention~(\textit{Whether}?), (2) takeover time  drivers~(\textit{When}?), and (3) takeover quality ~(\textit{How}?).  Due to the fact that resuming the control from the automated system requires visual, physical, and cognitive readiness, we focus on the multiple sources of information from the objective measurements of physiological responses to the subjective measurements, NDRTs, and vehicle trajectory to reliably predict the driver takeover time and takeover quality.


The primary phase of the framework is predicting \textit{whether} driver is intending to takeover, if the driver does not have the intention, estimation of the time and quality of takeover will not be proceeded. Once the system indicates a high chance of taking over, driver's takeover time~(\textit{when}) and quality of takeover~(\textit{how}) will be anticipated. Despite the recent studies on prediction of each individual phase of the driver's takeover performance~\cite{du2020predicting,lotz2018predicting,deo2019looking}, the obtained accuracy of their models were insufficient for practical implementation. Herein, we focus on developing a more practical solution that not only applies to all phases of proper takeover behavior, but also significantly outperforms the state-of-the-art results prediction of driver's takeover intention~\cite{guo2019predictive}, times~\cite{lotz2018predicting}, and the quality~\cite{deo2019looking}. Furthermore, as we establish a novel approach on prediction of driver's takeover behavior, we offer our novel framework configurations, implementation details, and source code to the Human-Computer Interactions (HCI) community to reproduce our obtained results~\footnote{Website is anonymized for the review purpose.}.  

% our proposed approach is shown to outperform the binary prediction of \textit{whether} the driver will takeover or not.
% Once the system could estimate the binary action of takeover, it will reliably predict the time and the quality of the driver's response.


We envision that our robust estimation of driver's takeover time and the takeover quality can be integrated into an intelligent vehicle safety system both for (1) AVs that use driver state in optimizing transfer of control decisions along with motion planning, and (2) assistive technology such as future advanced driver assistance systems (ADAS). By integrating DeepTake framework into the monitoring systems of the AVs, the automated system knows the potential category of driver's takeover behavior and can adapt its driving behaviour to match the drivers need. In addition, our novel approach provides a promising new direction for modeling driver's takeover time to lessen the effect of general and fixed design of TORs which considers homogeneous takeover time for all drivers. Our framework allows the AV to constantly monitors the category of takeover time and takeover quality of a driver and gradually adjust to match the need for proper takeover control.


% ~(i.e., either to takeover or not) as well as the time required to perform the necessary set of actions before takeover.
% However, there will also be cases where the AV’s ability to drive safely and to monitor its performance, is
% 2019). However, there will also be cases where the AV’s ability to drive safely and to monitor its performance, is
% impaired.



Therefore, we outline contributions of this work as follows:
\begin{enumerate}
    % \item \textbf{Scenario design:} We account for multiple critical types of transition requests including planned transfer of control with explicit alarm~(true alarm), nuisance alarm~(false alarm) accompanied by silent failure~(no alarm) of the automated vehicle to practically predict driver takeover behavior.
    \item \textbf{Novel approach:} To the best of our knowledge, our proposed DeepTake method is the novel prediction of the driver's reaction time and quality of takeover using multimodal data. Our DNN-based framework shows the driver’s reaction time and quality of takeover can be predicted as early as 10-sec prior to the initiation of TORs. Therefore, the automated system could gradually adjust the TOR timing to the needs of driver.
    \item \textbf{Feature contribution:} We provide evidence how the magnitude of certain features affecting the category of takeover reaction time and takeover quality. It presents a novel insight into the optimum number of features per modal for future advancement of on-road takeover response prediction. Our findings can be used to filtrating features and capture the most important features for takeover  behavior classification
    
    % \item We show how the driver's action-related features which are passively collected from the wearable devices along with vehicle trajectories can be used in predictive modeling to increase the individual-sensitivity in a timely manner. It can be the primary step towards personalizing TORs.
    % \item \textbf{Outperformance:} While prior studies in prediction of RT is missing, we qualitatively show that our model outperforms the state-of-the-art results under binary action of takeover prediction~\cite{du2020predicting} and the quality of the takeover~\cite{deo2019looking}.
    % \item \textbf{Open Source and Reproducibility:} As we establish a novel approach on prediction of driver's RT, we provide our novel framework configurations, implementation details,~and source code to the Human-Computer Interactions (HCI) community to reproduce our obtained results.  
    % \item We discuss the implications of our work on the design of future neural net facilities, including using the information gathered to enhance the chance of the correct prediction of human behavior. This can be integrated into many current systems to improve the automation safety.
\end{enumerate}

% The remainder of this paper is organized as follows. We begin by reviewing the related works, and present the details of our methodology followed by modeling framework. Using the obtained data and developed framework, we investigate prediction of binary takeover action and multi-class classification of driver reaction time.


==> DeepTakeArxiv/Sections/oldSections/MethodMotiv.tex <==


% What other studies have done?
% The majority of the studies have investigated the reaction time and and its relationship to the takeover quality in response to a TOR trigger. However, the recent automated accidents have shown that it is reasonable to expect that the automated system could fail to prompt TOR. Therefore, the automated system requires to constantly analyze the challenges and predict how the human's performance will be in an accurate and robust way using established sensor technology before triggering TORs.

AVs provide the underlying condition for users to have more free time to be engaged in NDRTs. Hence, their perception, and anticipation of incidents in the surrounding environment will be impaired until they have enough time to properly regain the situational awareness for a safe transition of control. A failure to reliably estimate the driver's cognitive and physical competence, situation awareness, and therefore takeover readiness before TOR, will cause anxiety to driver and potential tragic consequences to vehicle and its occupants. Thus, we propose DeepTake, an efficient multi-class DNN-based framework which accounts for continuous driver behavior monitoring by leveraging multimodal data including biometric sensors, NDRTs and engaged objects, vehicle dynamics, and subjective measurements, as illustrated in Figure~\ref{fig:llustrative}. 
It displays \textcolor{red}{our proposed DeepTake framework consisting of \textbf{four modules} dedicated to multimodal data collection, data preparation and feature extraction, DNN model, and classified takeover behavior outcomes.} Utilizing multimodal data fusion in our proposed DNN-based framework, helps more accurate and robust prediction of multiple phases of drivers’ takeover behavior~(\textit{where,when}, and~\textit{how}) than prior studies. DeepTake can help the automated system to adjust the TOR initiation to match drivers' takeover needs and ultimately help the driver to better prepared to safely navigate the incident for which the handover of control occurs. We explain each module of the DeepTake framework below.

\subsection{Multimodal data} \label{sec:Multimodal}
Figure~\ref{fig:llustrative} illustrates a user wearing biometric sensors showing changes in eye movement metrics accompanied by emotional responses while engaging with a ~\textcolor{red}{cellphone}. These non-intrusive, multimodal objective measurements detect driver's visual attention collected from eye-tracker, stress and anxiety through heart rate~(HR) and galvanic skin responses~(GSR). DeepTake framework incorporates wrist-type photoplethysmographic~(PPG) signals where its sensors' strap was wrapped around the participant's ring finger, while the GSR sensor straps was wrapped around the participant's index and middle finger~(See Figure~\ref{fig:llustrative}). Traditionally, driver status were only derived from the driving performance~(e.g., lateral and longitudinal control of the vehicle). However, since in the AVs drivers are no longer in control of the vehicle all the time, using wearable devices with big-data analytic can enable individualized measurement of driver's cognitive and physical states. Although we employed high-end sensors to precisely track driver's state changes, our intention were using physiological data as reliable features that future advancement of such system can be easily applied to real world applications. Below, we explain the subjective and objective multimodal measurements utilized in DeepTake framework indicating the drivers' visual attention, level of stress, and workload.


\subsubsection{Eye-tracker}
In automated vehicles, it is likely that drivers will engage with NDRTs. Eye-tracker captures eye-movement subsequent to shifting drivers visual attention before and after TOR. There is a high proven correlation between driver's eye movements and visual attention\cite{zeeb2015determines,wu2019assessing,alsaid2019moving}. In order to comprehend the attentiveness of driver to the surroundings environment before TOR, we acquired gaze coordinates, pupil diameters of each eye, fixation duration/sequence on the detected objects, and time to first fixation~(TTFF)~(see Table~\ref{tbl:data sources}). 
% One of the main components of eye-tracker is observation time which is calculated as the ratio between the fixation time and the time in which the object (e.g., pedestrian, truck, obstacle, etc.) appears in the visual frame. The smaller the ratio is, the less important (or not important at all) the object is to the driver or the driver failed to detect the object properly. 

\subsubsection{Heart Rate~(HR)} In a stressful driving context, variation of HR indicates the stress and affect situational awareness. DeepTake employs HR using photoplethysmographic~(PPG) signals recorded from
wearable Shimmer3 GSR+ device with a sampling frequency of 256Hz. PPG sensor monitors HR by emission of infrared light using LED into the body and measures the reflection back to estimate the blood flow. Unlike the electrocardiography~(ECG), PPG does not rely on the placement of metal electrodes on the participant's chest and can be found embedded in most smartwatches. Therefore, it not only provides us with the mobility required to gain uninterrupted information from the participants, but can also be practically employed as a result of requiring less intrusive body contact and maximized user experience. Fluctuation of heart rate in the time intervals between the nearby beats which occurs as a result of emotional factors can be measured by variability of heart rate~(HRV). HRV is the main parameter associated with detecting driver's workload~\cite{paxion2014mental}, driver's stress~\cite{dillen2020keep}, and driver's drowsiness~\cite{vicente2011detection}. In this study we extract features from HRV analysis for monitoring driver's readiness. 



\subsubsection{Galvanic Skin Responses~(GSR)} 
Another physiological data considered in this study is GSR, which simply indicates the conduction ability of the skin~\cite{dillen2020keep,nourbakhsh2012using}. As skin conductance is balanced by sweat secretion caused by sudomotor activity, any action accounting for muscle activation like stress can be objectified by GSR~\cite{braithwaite2013guide}. Therefore, in the context of driving any emotional arousal~(e.g. startle response, sudden fear, and stress), the magnitude of the electrical resistance of the skin decreases, while the conductance increases. Along with HR parameters, GSR has been proven as one of the most valid indicators of stress and workload of a drivers~\cite{dillen2020keep,foy2018mental,mehler2012sensitivity,radlmayr2014traffic}. Thus, it was used to monitor the objective stress level of drivers. 


\subsubsection{NASA-Task Load Index~(NASA-TLX)}
In order to complementing the objective measurements, we also use NASA-TLX as one of the most extensively exploited objective metrics for the measurement of driver's workload. We use NASA-TLX at the beginning of each trial to prevent participants become annoyed to rate their workload while driving. It provides ratings methods, on a scale with 21 gradations, across six critical domains for proper reaction in driving: mental demand, physical demand, temporal demand, performance, effort, and frustration.

\subsubsection{PSS-10.}
The 10‐item Perceived Stress Scale~(PSS‐10) is another subjective metric developed to measure perceived psychological stress or \textit{"stress-related components of unpredictable, uncontrollable, and overloading life events”}\cite{iseland2018exploratory} over the past 30 days. We only obtained this result once at the beginning of the driving session.


\subsubsection{Non-Driving Related Tasks~(NDRTs)}
AVs provide environments where drivers can interact with various NDRTs, such as reading books or using smartphones. These NDRTs play a crucial role in the acceptance of the automated vehicle. Each driving task, however, requires a certain level of visual, physical and cognitive demand. We selected the most common NDRTs herein to create realistic scenarios by which drivers would be most likely to engage in the AVs~\cite{gerber2020self,dogan2019effects}. These selected NRDTs include Reading, simple arithmetic problem solving questions, Browsing the Internet, and Conversation. These tasks were not only chosen to suit our experiments' setup~(see Figure~\ref{fig:simulator}), but also to follow the framework of difficulty level in flow theory~\cite{csikszentmihalyi1990flow}. The reading and arithmetic problem solving questions tasks have two main difficulty levels~(easy and medium adapted from\cite{nourbakhsh2012using} which reported strong correlation between the questions and physiological responses). 

\subsubsection{{Vehicle dynamics}}
From the vehicle dynamics data we capture the angle of the steering wheel, accelerator and brake pedals, distance from the neighbor lanes, distance to hazard, and finally the speed of the car. These features display the instantaneous driver's reactions in order to control the vehicle appropriately. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%===============================================
%%%%%%%%%%% Framework Graph %%%%%%%%%%% 

% \begin{figure*}[h!]
%   \centering
%   \includegraphics[width=5.2in]{Figures/NN_Structure_3.png}
%   \caption{The proposed DeepTake framework for the prediction of driver's takeover behavior based on a deep learning architecture. This framework includes four steps of multimodal data collection, data preparation and feature extraction, DNN model, and classified takeover behavior outcome. The input of the framework is the driver-related signals, vehicle dynamics information, subjective measurements, and the non driving-related tasks. The 10sec time window is selected where all the multimodal data is fused to feed into the DNN model. The output layer shows the three defined classes for the prediction of takeover(either takeover time or quality.)}
%   \label{fig: NN_Architecture}
% \end{figure*} 
%%%%%%%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Data preparation and feature extraction}\label{sec:Dataprep}
The wide range of a driver's action related features provides a better chance to draw insights into different types of driver's takeover behavior. However, the larger the number of features, the harder it is for the classification algorithm to build a comprehensive model from the obtained data, especially considering the smaller number of participants proportional to the number of features. Therefore, we initially prepare and extract the utmost features from all of the aforementioned modalities, then applied feature selection methods to reduce the number of features to a set that is representative of our data. 

As introduced in section~\ref{sec:Multimodal}, multimodal data including driver physiological signals from wearable devices, NDRTs, subjective measurements, and  vehicle dynamics were acquired. At this step of the DeepTake framework, the captured signals are filtered and meaningful features are extracted. This step aims to fuse all the multimodal data into a joint representation to feed into the next step of DNN model~(see Figure~\ref{fig: NN_Architecture}). Since DeepTake covers three \textcolor{red}{phases} of takeover behavior~(\textit{where, when,} and \textit{how}), the selected features need to expose all the three phases together to reliably guide the automated system about the driver's status. Therefore, features should be carefully and elaborately extracted, then selected. In order to do so, the primary essential step is finding an appropriate time window size. We applied fixed window method wherein the segmented windows will get the same labels as the original. Studies have found that 10 second is an adequate time budget for a driver to react properly\cite{walch2017car,zeeb2015determines}. Thus, we selected all of the following features over the 10sec fixed time window before the moment of takeover alarm. Within the segmented window, we preprocess and extract meaningful features from the physiological data. As the varying forms of signal used in DeepTake framework, we took the approach suitable for each individual signal. Our approach for identifying relevant and informative features is exploratory and based on previous research.


%===============================================
%%%%%%%%%%% List of Features %%%%%%%%%%% 

% Table for Features list
\vspace{-1mm}
\input{Tables/Features_list}
\vspace{-1mm}

%===============================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Feature Extraction}}

\paragraph{\textbf{PPG}}
As it is suggested by~\cite{singh2013comparative}, a min-max normalization was executed on PPG signals prior to pre-processing and feature extraction. We applied the min-max normalization on a 10second window of the baseline scenario as follows:

\begin{equation} \label{eq:Min-Max Normalization}
    S_{norm} =\frac{PPG_{raw} -\min(PPG_{raw})}{\max(PPG_{raw})-\min(PPG_{raw})}
\end{equation}

where $S_{norm}$ represents the normalized PPG signal. The normalized PPG signals were then filtered by applying a 2\nd order Butterworth high pass filter with a cut-off of 0.5Hz followed by a 1\st order Butterworth low pass filter with a cut-off frequency of 6Hz. The filtering procedure can be defined as: 

\begin{equation} \label{eq:Min-Max Normalization}
    S_p = f_{b}(S_{norm}, c_l, c_u)
\end{equation}

where $S_p$ represents the pre-processed signal and $c_l$ and $c_u$ show the lower and upper bound cutoffs, respectively. 
We used HeartPy, an open-source toolkit analyzing PPG data, for filtering and extracting the following features\cite{van2019heartpy}.

In this study we also extracted HRV assoiciated features from the preprocessed PPG signal~($S_p$)~and focused on the most common time-domain indices of HRV by which we could quantify the amount of HRV after receiving TOR. The extracted features used in this study include the standard deviation of normal beats~(SDNN), root mean square of successive differences between normal heartbeats~(RMSSD), and Percentage of the number of sequential normal beats differences that are over 50 ms~(pNN50). 

\paragraph{\textbf{GSR}}
For each TOR, GSR features were extracted from the part of the signal corresponding to 10second prior TOR. Important features extracted from skin conductance are 1)~the quantity of peaks and, 2)~the peak amplitude~\cite{manawadu2018tactical,nourbakhsh2012using}. A peak occurs when a subject gets a phasic response higher than the baseline of skin conductance~(the GSR signal contains phasic and tonic components and in this study we only use features extracted from the phasic component). The GSR peak amplitude is a measure of how far above the baseline the peak occurred. In other words, amplitude is the difference between the value of local maximum and the point the signal starts to rise.





\subsubsection{\textbf{Feature Selection}}\\
% feature selection
% and combination is another obstacle for accurate takeover behavior classification
To prepare the features for the DNN model, the sliding window of 10 sec was exploited to individual feature from each modality~(more details in sec~\ref{sec:Dataprep}. We included all of the data sources as we could possibly obtain and later acquired meaningful features from the multimodal data sources. To remove individual-dependency of the wearable signals, we normalized the features reported in Table~\ref{tbl:data sources} by Z-score normalization technique, except for PPG signals which we used min-max normalized. Finally, we reached more than 75 features, which is too many for the amount of data we had. Thus, we removed the features with no variation or a large amount of missing values~(more than 50\%). For features which passed this filtering process and still had missing values, their missing values were imputed with their mean values. We executed a correlation analysis on the feature set to identify features that are highly correlated with each other and therefore redundant with no discriminatory power to infer the driver's reaction time categories. This unbiased and compact set of features was selected using two feature selection methods: Least Absolute Shrinkage and Selection Operator~(LASSO) and Random Forests. We used LASSO to select a subset of features that are nearly independent and eliminate irrelevant variables to the driver's reaction time. LASSO performs well in selecting a stable set of features and tends to select one feature among highly correlated features, resulting in a reduction of features. Random Forests on the other hand rank all of the features based on their importance for the classification of reaction time. The overlapped features chosen by the two methods were utilized to develop the final classification model of reaction time.

Let the explanatory selected features be denoted as
$X= \{x_1, x_2,...,x_d\}$, where X is the set of pre-processed features we could pass X into our proposed neural net. The final features extracted and used in the model are shown in Table~\ref{tbl:data sources}. The intersection of the feature selection methods incorporated 35 features. Note that one-hot encoder was used to handle the categorical features which increase the number of columns for training the model.

% To prepare the data for the CNN architecture, the sliding win- dow strategy was applied to each low level feature from each modality. Using sliding window strategy, the signals are segmented into a fixed window size. The segmented windows are the new training data and will get the same labels as the original trials
\subsection{Target Labeling}
We used features listed in Table~\ref{tbl:data sources} to feed to the DNN model to predict driver takeover behavior including \textit{intention}, \textit{time} and \textit{quality}. Previous studies defined the labels objectively through asking multiple humans to watch and rate the driver's performance~\cite{deo2019looking,du2020predicting}.
However, the key for practical application is subjectively selecting thresholds for acquiring the target labels. Thus, we define the takeover intention, time and quality labels for DeepTake framework as follow.

\subsubsection{Takeover Intention}
The takeover intention is a binary action of whether the driver is willing to takeover or not. Therefore, once the driver initiates the action of resuming the control by pressing the two buttons mounted on the steering wheel~(see Figure~\ref{fig:simulator})the multimodal data are labeled as \textit{takeover}, otherwise \textit{not-takeover}.

\subsubsection{Takeover Time}
While driving the AVs, the system initiates the TOR ($t_{alarm}$), drivers should regain the situational awareness and assess the scene for the necessity of taking over. If the driver quickly observes the situation and decides that the current lane is not safe, she is obligated to maneuver the vehicle safely. The moment of taking over or the starting time of manually controlling the vehicle is defined as $t_{takeover}$~\cite{sadeghian2018feel,gold2015utilization}. The $t_{takeover}$ is defined as the first contact with the steering wheel/pedals~\cite{zeeb2015determines} or pressing the takeover buttons~\cite{kim2017takeover}. In our driving simulator environment, once the participant assumes control by simultaneously pressing two assigned buttons on the steering wheel~(more details in sec~\ref{sec:Procedure}). Thus, the value of \textit{reaction time~(RT)} was calculated as:
\begin{equation} \label{eq: reaction time}
    \centering
    \textit{RT} = t_{takeover} - t_{alarm}
\end{equation}

The time interval between the TOR and the completion of the transition to manual driving is RT~(see Figure~\ref{fig:Scenario}). Subsequently, with the intention of creating multi-classes of reaction time, we modified reaction time into \textit{three} and \textit{five classes}. The  thresholds for each class of RT complies the existing lines of research in pre-defined i\textsuperscript{th} percentile of RT~\cite{coley2009driver} where three-class of RT is thereby classified as: low-~($RT <2.6sec$ ), medium-~( $2.6sec \leq RT \leq 6.1sec$), and high-~($6.1sec <~RT$) reaction time. This led us to even narrower five-class classifications of reaction time in which each class is defined as: lowest-~(RT < $1.5sec$), low-~($1.5sec \leq RT < 2.6sec$), medium-~($2.6sec \leq RT < 4.7sec$), high-~($4.7sec \leq RT \leq 6.1sec$), highest-~($6.1sec < ~RT$).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Takeover Quality}
Driver reaction time is how prepared the driver is to take the control, whereas the quality is defined by the occurrence of driving errors such as lane exceedances, insufficient securing or inadequate speed. Thus, the takeover quality is measuring how safe the driver's maneuver the control of the car. The performance metrics for evaluating this matter is either based on braking or steering performance~\cite{happee2017take}.In this study, we apply the latter metric where variability of vehicle position is used to infer how well the driver takeover.  low-~($position <3.5m$ ), medium-~( $3.5m \leq position \leq 7m$), and high-~($7m <~position$) takeover quality.

\subsubsection{Fusion} Due to the varying modalitis collected in this study and signal complexity driven by underlying preprocessing and feature extraction, extracted features~(Table.\ref{tbl:data sources}) are combined into one vector to use into the DNN model.


%%%%%% Driving Simulator %%%%%%%%%%%%%%%%
% \textcolor{blue}{
% Driver takeover and reaction time was studied with the use of a driving simulator. The main advantage of utilizing any driving simulator is not only creating all possible driving scenarios which drivers may or may not encounter daily, but also collecting vehicle information such as speed, lateral and longitudinal positions which may not be easily feasible in the field. Besides, we could safely collect subjective detailed measurements of drivers through various surveys. All the aforementioned benefits can be used as the features for developing a robust framework for predicting driver reaction time.}







% \textcolor{blue}{
% %-------------------
% % WHY DNN or ML?
% Automated systems tend to minimize the intervention rate but they are still unequipped to tackle several sudden events~\cite{favaro2018autonomous} and therefore rely on human's abilities to assist~\cite{seppelt2019keeping}. Nevertheless, as the automated systems alter the driver's performance, they have a greater difficulty in safely controlling the automated vehicle, due to substantially losing situational awareness~\cite{merat2014transition}. 
% % Given adequate time, however, their performance improves~\cite{gold2018modeling}.
% While automation behavior can be predicted to some \todo{extent}, human behavior is inherently stochastic and conditioned to a determined situation. This makes predicting human behavior difficult and crucial to combat. Fortunately, the recent rapid advancement of DNN techniques equipped with enough data shows stellar reliability for modelling human behavior~\cite{kim2020fundamentals}.
% Much research has focused on understanding different aspects of the reaction time such as the time gap needed for drivers to react properly and statistical analysis of drivers reaction time. However, a few studies have focused on providing a cohesive, holistic framework by which the system could decide the human driver is prepared enough to safely takeover. Our framework provides the fundamentals for a system to reliably predict the drivers reaction time and quality of takeover based on their performance history through using Deep Learning.}



% \textcolor{red}{Why NDRTs}
% Conditionally automated driving and the engagement in NDRTs represents a novel situation for a driver, in which drivers have more free time to the task they desire to. In such situation, the future of mobility will depend on the constructive collaboration between human and the automated system. In this study we aim to provide the opportunity not to limit driver access to NDRTs, but to provide enough time for driver to adjust the situation to takeover when it's needed. Although the in-lab setup was used due to the fact that it is nearly impossible to collect enough driver reaction time data before dangerous events with the conventional in-car data collection protocol and safety concern,the presented framework can impact on how humans would interact with automated vehicle. The in-lab setting provided some of the most common tasks which may drivers will interaction with while riding.

% \textcolor{red}{BigPicture:}
% When the automated system evaluates whether a non-controllable event could happen and the situation might be safety-critical it will assess the situation of driver to take-over the control. To assess the driver status, there are two factors that a system needs to evaluate before relinquishing the control in a timely manner: 1) Driver’s reaction time, 2) Quality of takeover
% Driver reaction time is how prepared the driver is to take the control where as the quality is defined by the occurrence of driving errors such as lane exceedances, insufficient securing or inadequate speed. The correct and reliable judgment of driver status could be life-saving which lead to higher performance to be near perfect.  \\



==> DeepTakeArxiv/Sections/oldSections/Modeling.tex <==

This section presents the multimodal DNN architecture of DeepTake framework. Figure~\ref{fig: NN_Architecture} shows the steps of DeepTake framework for the classification of multi-class takeover behavior. We described how the signals were processed followed by features extraction in Sec.\ref{sec:Dataprep}. In this step, we fuse the extracted multimodal features to build a DNN model to detect binary class of driver's takeover intention~(whether), three classes of takeover time~(when), and three classes of takeover quality~(how). 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}[t!]
% \caption{Train a neural network with mini-batch stochastic gradient descent}
% \begin{algorithmic}[1] \label{alg:NN}
% \STATE   $X,y \gets  Preprocess (x,y)$
% \STATE  Upsampling~$(X,y)$   
% \STATE initialize($net$)
% %\STATE Split~(train,test)
%     \FOR{ epoch $= 1,...,K $}
%         \FOR{ batch = 1,...,b}
%         \STATE validation = $0.1$
%               \STATE  $z \gets$ forward$(net, X)$
%               \STATE $ \ell \gets$ loss$(z, y)$
%               \STATE $grad \gets$ backward($\ell$)
%               \STATE update($net, grad$)
%         \ENDFOR
%     \ENDFOR
% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Classification}\label{sec:classifications}
In order to implement a framework in the real world, we should first and foremost assure the safety of the users by using methods with the highest reliability. Prediction of each individual phase of takeover behavior, intention, time and quality, has been studied but they have not been able to achieve a relatively high accuracy. Comparing the results of takeover intention binary classification,  provides the confidence in our selected features to tackle a more challenging problem of multi-class classification of takeover time and quality using the same features. We applied our selected features into multiple machine learning algorithms to compare their performances in all three phases of takeover. Our process of choosing the learning algorithms is an exploratory task with trials and tests of multiple off-the-shelf algorithms~(see Table~\ref{tbl:results comparison}) and choosing those that perform the best. We evaluate the performance of Logistic Regression, Gradient Boosting, Random Forest,  Bayesian Network, Adaptive Boosting~(Adaboost), and Regularized Greedy Forest~(RGF). RGF with Adaboost provide the best performance according to our evaluation criteria explained below.


\subsubsection{Neural Network Architecture}
DeepTake utilizes feed-forward DNN with mini-batch stochastic gradient descent. This DNN structure begins with an input layer to match the input features and each layer receives the input values from the prior layer and outputs to the next one~(see Figure~\ref{fig: NN_Architecture}). DNN provides the flexibility to process the inputs independently so that it fits feature complexity. The DNN in this study includes three hidden layers with 23, 14, and 8 \textit{ReLu} units respectively in hidden layers. As the main purpose of this paper is to develop a model for multi-class classification of driver takeover behavior, the output layer of DNN consists of three \textit{Softmax} units representing three takeover time and quality classes~(low-, medium-, and high-). Therefore, our implemented DNN uses ReLU~(equation \ref{eq:Relu funciton}) as an activation function in each hidden layer and uses the Softmax~(equation \ref{eq:Softmax funciton}) function as the classification function at the last layer of the network.

\begin{equation} \label{eq:Relu funciton}
    f(x) = max(0,x)
\end{equation}

\begin{equation} \label{eq:Softmax funciton}
    \sigma(z)_j = \frac{e^{z_j}}{\sum_{k=1}^k e^{z_k}} \\~, \forall j \in\{1,...,k\}
\end{equation}

We used Softmax cross-entropy loss with an Adam optimizer with a learning rate of 0.001 to update our parameters and trained our DNN model over 400 epochs. In each iteration, we randomly sampled a batch of data in order to compute the gradients with a batch size of 30~($b=30$). Once the gradients were computed, the initiated parameters got updated. It automatically stops after 400 passes through the dataset. The early stopping method throughout the training procedure prevented overfitting.




==> DeepTakeArxiv/Sections/oldSections/Results.tex <==
%%%%%%%%%%% Accuracy Vs Loss %%%%%%%%%%% 
\begin{figure}[t!]
\centering
   \includegraphics[width=\textwidth]{Figures/ROC_3RT_Quality.png}
   \caption{a) The ROC curve of six machine learning algorithms employed for classification of takeover. ROC curve shows the average performance of each classifier and the shadowed areas represent the 95\% confidence interval.  The AUC value of 0.5 refers to a random classifier. In the legend, the AUC associated with each classifier is shown. b)\textcolor{red}{change the caption}}
   \label{fig:ROC}
\end{figure} 
%%%%%%


%%%%%%%%%%% Table for model comparison %%%%%%%%%%%%%%%%%%%%%%
\vspace{1mm}
\input{Tables/Model_Comparision}
\vspace{0.1mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As the prediction of driver reaction time is contingent upon the driver's decision to take over from the autonomous systems after receiving TOR, we had to predict whether drivers were able to take over or not. Although takeover prediction has been recently studied~\cite{du2020predicting,braunagel2017ready}, it still needs an extensive improvement to be practical and integrated into an automated system. Our extracted features contributed to a higher prediction accuracy in the binary classification of takeover. The results show~(Table~\ref{tbl:results comparison}) that RGF attains the highest accuracy and weighted F1 score~(92\% and 89\%) followed by AdaBoost~(88\% and 88\%) and Logistic Regression~(77\% and 88\%). Moreover, ROC was applied in order to better evaluate each of the classifiers. Figure~\ref{fig:ROC} shows ROC curves and AUC values for all six machine learning models to infer the binary action of takeover. RGF showed the best classification performance with an AUC of 0.94. Similar to accuracy level, AdaBoost had a slightly lower performance with an AUC= 0.91. The AUC values provided in Figure~\ref{fig:ROC} can be interpreted as the probability of  correctly classifying the driver takeover into the candidate category is higher than randomly selecting takeover or not-takeover~(red line in Figure~\ref{fig:ROC}). Table~\ref{tbl:results comparison} together with the results obtained from the AUC in Figure~\ref{fig:ROC} ensure that our selected features with the right classifier surpass the takeover prediction of previous studies. 

Therefore, a better performance in takeover detection achieved through the machine learning algorithms~(see Table \ref{tbl:results comparison}) led us to a multi-class prediction of driver reaction time. As some of the machine learning algorithms attained high accuracy in binary classification of takeover, their performances along with our developed DNN in classifying multi-class classification of reaction time would show the robustness of the model.

For the training of our DNN, 70\% of the data was used and the rest was assigned equally for the testing and validation. As explained in \textcolor{red}{Algorithm~\ref{alg:NN}}, in order to satisfy the imbalanced data in each category, data in the minority classes were required to be upsampled. Due to the size of the dataset, the processing of each epoch lasted 570 seconds, that is, in comparison with the other tests, the computational effort was increased to generate a more robust model.


%%%%%%%%%%% Accuracy Vs Loss %%%%%%%%%%% 
\begin{figure*}[t!]
\centering
   \includegraphics[width=5.5in]{Figures/Accuracy_vs_Loss.pdf}
   \caption{The left figure shows the accuracy result of training and test sets for 400 epochs whereas the right figure indicates the loss for our DNN model on prediction of three class driver's reaction time.}
   \label{fig:Model_Accuracy_vs_Loss}
\end{figure*} 
%%%%%%

Table~\ref{tbl:results comparison} compares our DNN model with other classifier algorithms. It is evident that our DNN outperforms all of the classic algorithms. In three-class classification of reaction time~(low,~mid,~high), the DNN model achieves a weighted-F1 score of 0.87, thereby achieving the best performance on this task by a substantially better accuracy result of 92.3\%. As shown in Figure~\ref{fig:Model_Accuracy_vs_Loss}, DNN gained a high accuracy for both the learning and testing sets. However, the model did not significantly improve and stayed around 92\% accuracy after the epoch 250. Among the classifiers, though, RGF and AdaBoost still performed better~(73.4\% and 64.1\%).

In the five-class classification of reaction time, the results on the validation set show that DNN model also outperformed~(around 12\% more than RGF and 115\% better than RandomForest) the standard machine learning classifiers with respect to weighted F1- score and accuracy. As shown in Table~\ref{tbl:results comparison}, the performance of each model varied regardless of the number of classes. But, similar to three-class classification, the RGF model achieved the best performance~(66.4\% accuracy) on the five-class distinction of reaction time among the six machine learning algorithms. The other algorithms achieved lower performance than the RGF model.


%%%%%%%%%%% Confusion Matrix 3_Class %%%%%%%%%%% 
\begin{figure}[h!]
\centering
  \includegraphics[width=0.48\textwidth]{Figures/CM_ThreeCL_RT.png}
  \caption{Confusion matrix for the prediction of three classes of driver's takeover time.}
  \label{fig:CM-ThreeClass}
\end{figure}
%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 

To capture a better view of the performance of our DNN model on reaction time prediction, we computed the confusion matrix for each multi-class classification problem. Figure~\ref{fig:CM-ThreeClass} displays the performance of our DNN model as the best classifier of three-class reaction time. As the diagonal shows the number of correctly classified, it can be seen that the misclassification in each class is small. The lowest true positive number is achieved by the medium reaction time class. Also, marginal misclassifications are found in the 1\%-2\% of the low and high reaction time label. Overall, the DNN model obtains good performances in correctly classifying the three-class reaction time.

Figure~\ref{fig:CM-FiveClass} represents the performance of DNN on classifying the five-class reaction time. Although DNN was not as distinctive in five-class classification as in the three-class, it still achieved satisfactory results. Lowest, low and medium reaction times are the top three pairs that were the most frequently misclassified by the DNN algorithm. The reason might be that the selected features do not have the required distinctive characteristics to perfectly divide the low and medium reaction times. In each class, however, it could still distinguish between four other classes with an average of 70\%. 


%%%%%%%%%%% Confusion Matrix 5_Class %%%%%%%%%%% 
\begin{figure}[h!]
\centering
  \includegraphics[width=0.48\textwidth]{Figures/CM_FiveCL_RT.png}
  \caption{Confusion matrix for the prediction of five classes of driver takeover time.}
  \label{fig:CM-FiveClass}
\end{figure}
%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 


\subsection{\textcolor{red}{Takeover Quality w.r.t position}}


==> DeepTakeArxiv/Tables/Features_list.tex <==

%===============================================
%%%%%%%%%%% List of Features %%%%%%%%%%% 
\begin{table}[t!]
\small\addtolength{\tabcolsep}{-3pt}
  \begin{center}
    \caption{List of extracted features used in DeepTake}
    \label{tbl:data sources}
    \begin{tabular}{c| c c c}
      \toprule % <-- Toprule here
        \textbf{Data Source} & \textbf{Feature } & \textbf{Type} & \textbf{Values} \\
        \hline \hline
         \multirow{5}{*}{Eye movement} 
         & Gaze position & float & (1920$\times$1080) \\
          & Pupil size & float & (0-7) \\ 
          & Time to first fixation & int & (1-90) \\ 
          & Fixation duration & float & (100-1500ms) \\
          & Fixation sequence & int & (1-2500) \\
          \hline
          \multirow{3}{*}{Heart rate~(PPG signal)}  
          & SDNN & float & (45-75ms) \\
          & RMSSD & float & (25-43ms)\\
          & pNN50 & float & (18-28\%)\\
          \hline 
          \multirow{2}{*}{GSR signal} 
          & Number of peaks & int & (1-6)\\
          & Amplitude of peaks & float & (0.01- 1.58µs) \\
          \hline
        \multirow{3}{*}{Pre-driving survey}
          & Gender & binary & (M-W)\\
          & NASA-TLX & categorical & (1-21) \\
          & PSS-10 & categorical & (0-4)\\
           \hline
        \multirow{1}{*}{Secondary tasks}
          & NDRTs & categorical & (C,U,R,S)$^{1}$\\
          \hline
        \multirow{7}{*}{Vehicle data}        
          & Right lane distance & float & (0.73-2.4m) \\
          & Left lane distance & float & (1.02-2.8m) \\
          & Distance to hazard & float & (98-131m) \\
          & Steering wheel angle & float & (-180-114$^{\circ}$)\\
          & Throttle pedal angle & float & (15-21$^{\circ}$) \\
          & Brake pedal angle & float & (0-17$^{\circ}$) \\
          & Velocity & float & (0-55mph) \\
         
     \bottomrule % <-- Bottomrule here
    \end{tabular}
  \end{center}
   {\scriptsize 1:~\textit{C}; Conversation, \textit{U}; Using cellphone, \textit{R}; Reading articles on tablet,~and
   \textit{S}: Solving arithmetic questions}
\end{table}



==> DeepTakeArxiv/Tables/Model_Comparision.tex <==


%%%%%%
%%%%%%%%%%% Prediction results %%%%%%%%%%% 
\begin{table}[b!]
\small\addtolength{\tabcolsep}{-3pt}
  \begin{center}
    \caption{Classification performance comparison.}
    \label{tbl:results comparison}
    \begin{tabular}{l|l| c c}
      \toprule % <-- Toprule here
        \textbf{Target value} & \textbf{Classifier } & \textbf{Accuracy} & \textbf{W-F1$^{1}$ score} \\
        \hline \hline
          \multirow{7}{*}{\shortstack{Takeover Intention}}
          & Logistic Regression & 0.77& 0.81  \\
          & Gradient Boosting & 0.76 & 0.75 \\
          & RF$^{2}$ & 0.75 & 0.72 \\
          & Naive Bayes & 0.71 & 0.66 \\
          & Ada Boost & 0.88 & 0.87 \\
          & RGF$^{3}$ & 0.92 & 0.89 \\
          &\textbf{DeepTake} & \textbf{0.96} & \textbf{0.93} \\
         
        \hline
         \multirow{7}{*}{Takeover Time}
          & Logistic Regression & 0.47& 0.45\\
          & Gradient Boosting & 0.47 & 0.46 \\
          & RF & 0.44 & 0.45 \\
          & Naive Bayes & 0.36 & 0.38 \\
          & Ada Boost & 0.64 & 0.58 \\
          & RGF & 0.73 & 0.71 \\
          & \textbf{DeepTake} &\textbf{0.93} & \textbf{0.87} \\
          \hline 
          \multirow{7}{*}{Takeover Quality}
          & Logistic Regression & 0.65 & 0.63\\
          & Gradient Boosting & 0.60 & 0.59 \\
          & RF & 0.53 & 0.52 \\
          & Naive Bayes & 0.41 & 0.39 \\
          & Ada Boost & 0.42 & 0.39 \\
          & RGF & 0.82 & 0.77 \\
          & \textbf{DeepTake} &\textbf{0.83} & \textbf{0.78}\\
     \bottomrule % <-- Bottomrule here
    \end{tabular}
  \end{center}
{\scriptsize 1: \textit{Weighted F1-score};
2:\textit{Random Forest};
3:\textit{Regularized Greedy Forests}} 
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> DeepTakeArxiv/Tables/NDRTs.tex <==

\setlength{\abovecaptionskip}{-0.5pt}
\setlength{\belowcaptionskip}{-2pt}
\setlength\intextsep{1pt}
%%%%%%%%%%% NDRT Table
\begin{table}[t!]
\begin{center}
 \small\addtolength{\tabcolsep}{-2pt}
    
    \caption{Non-driving related tasks (NDRTs) used in our study} 
    \scalebox{0.74}{
    \label{tbl:SecondaryTasks} 
    \begin{tabular}{l|l}
        \toprule 
         \textbf{Task Type} & \textbf{Definition} \\
        \hline
        \hline
        Conversation with passenger & Interacting with the experimenter who sits close to the participants\\
        \hline
        Using cellphone & Interacting with their cellphones for texting and browsing\\
        \hline
        Reading articles & Reading three types of articles (i.e.easy,mid,hard) on the tablet \\
        \hline
        Solving questions & Answering 2-level arithmetic questions (i.e. easy and medium) \\
        \bottomrule
    \end{tabular}}
    \end{center}
\end{table}
%%%%%%%%%%%%%%

==> DeepTakeArxiv/Tables/TOR_Modalities.tex <==
\begin{table}[h!]
\small\addtolength{\tabcolsep}{-5pt}
  \begin{center}
    \caption{Takeover request modalities}
    \label{tbl:TOR_Modalities}
    \begin{tabular}{l| p{60mm}}
      \toprule % <-- Toprule here
      \textbf{Types of TOR} &
      \textbf{Explanation}\\
      \hline \hline
      False Alarm~(FA)  & Takeover request in the situation where it is safely managed or wrongly recognized \cite{naujoks2014effect}\\
     \hline
      No Alarm~(NA)  & Not initiating Takeover request in the situation that is needed\\
      \hline
      True Alarm~(TA) & Correctly initiating Takeover request in the situation that is needed\\
     \bottomrule % <-- Bottomrule here
    \end{tabular}
%{\scriptsize 1: \textit{Number of repetitions for each type of alarm.}}
  \end{center}
\end{table}

==> Figures/Illustrative_figure.tex <==

 
 %%%%%%
\begin{figure*}[h!]
   \centering
   \includegraphics[ width=\columnwidth]{Figures/DeepTake-overview-revised.png}
   \caption{DeepTake uses data from multiple sources (pre-driving survey, vehicle data, non-driving related tasks~(NDRTs) information, and driver biometrics) and feeds the preprocessed extracted features into deep neural network models for the prediction of takeover intention, time and quality.}
   \label{fig:llustrative}
\end{figure*} 
%%%%%%

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> Sections/oldSections/Introduction.tex <==

Automated vehicles~(AVs)~\cite{sae2018taxonomy}) have been introduced with the aim of rapidly improving functionality, to the degree that highly automated driving will be introduced to the general public within the next few years. Audi’s traffic jam pilot, Tesla’s Autopilot, Mercedes' Distronic Plus are only a few examples of such commercially available vehicles~\cite{boelhouwer2019turmoil,menzel2018scenarios}. AVs let drivers take their hands off the wheel and their attention away from the primary task of driving~\cite{nhtsa2013department,mccall2019taxonomy}.  However, there are still challenging scenarios for AVs to safely maneuver wherein human should backup~(e.g., country roads with poorly visible lane markings, and other unfamiliar incidents)~\cite{banks2018driver,louw2017coming}. To cope with AVs' needs for constructive collaboration with human, we present DeepTake, a deep neural network~(DNN)-based framework for robust prediction of drivers' takeover behavior using multimodal data.

Despite automated systems have seen undeniable advances in the recent years, the commonality of their human-automation interaction design has not been thoroughly adapted to the new role of the driver as a fallback ready~\cite{tenhundfeld2020trust,hancock2019future,endsley2017here}. As we may be many years away from the fully-automated vehicles which can replace conventional, human-driven vehicles, it is important that the automated system constantly estimates how receptive the human is to the hazardous situations as early as possible to the extent of being able to takeover control from the automated system in a safe manner. This will potentially alleviate the safety concerns associated with the driver's status, engaged in non-driving-related tasks (NDRTs), inattentive, and fatigued, prior to takeover the vehicle control.

Currently, the Society of Automotive Engineers~(SAE) dictates that drivers need to be available to intervene when a transition to driver is crucial based on preset requirements or limitations in the automated system~\cite{lee2018perspectives,endsley1995out}. In this transition, the automated system prompts the driver concerning the vehicle status and asks to relinquish control~(takeover request or TOR) of the vehicle to the driver~\cite{bazilinskyy2017usefulness}. This requires drivers to takeover from the automated system in a given limited time~\cite{zeeb2016take}. However, shifting the role from a passive monitor who may have engaged with NDRTs for a prolonged time to an active controller in a timely manner may in fact leave the driver in a less capable state to make life-saving decisions. 
% But, what would happen if the automated system estimates how long the driver would take to resume and safely control the vehicle~(e.g., more than the time to collide)?
% Explain the need and how we solve it
Furthermore, overloaded, tired, and distracted drivers may need more time than their normal conditions to respond properly and the system needs to facilitate it by predicting driver's status before initiating TOR. 

Transitioning to manual control introduces two challenges for proper takeover performance: (1)~\textit{when} human will be able to takeover~\cite{eriksson2017takeover,zeeb2016take}, and (2)~\textit{how} adequately safe human will regain the control~\cite{happee2017take}. The safety countermeasures or \textit{"takeover quality"} is relatively interconnected to timing of the reaction as the longer reaction time to a TOR may increase the chance of proper controlling of the vehicle~\cite{louw2017coming,gold2013take}. Nevertheless, the driver's reaction time and the relevance of takeover quality depends on the contextual environment, the vehicle's and driver's status. Therefore, robust prediction of \textit{when} and \textit{how} human performs takeover is critically challenging for safe and timely transfer of control. 




%  Therefore, there is a need for a data driven monitoring system which reliably predicts drivers reaction time and the possible quality of takeover.

% it may not request human interference until the driver is fully capable of doing so. This paper develops a novel framework for the prediction of the driver's reaction time using Deep Neural Network~(DNN). 
% To the best of our knowledge, this is the first DNN-based model which extracts features from multiple wearable sensors along with vehicle trajectory information to perform reaction time classification. 


To address the above challenges, we present a framework utilizing multiple sources of information to reliably estimate three phases of driver's takeover behavior before initiating TORs. Our framework predicts driver's: (1) takeover intention~(\textit{Whether}?), (2) takeover time  drivers~(\textit{When}?), and (3) takeover quality ~(\textit{How}?).  Due to the fact that resuming the control from the automated system requires visual, physical, and cognitive readiness, we focus on the multiple sources of information from the objective measurements of physiological responses to the subjective measurements, NDRTs, and vehicle trajectory to reliably predict the driver takeover time and takeover quality.


The primary phase of the framework is predicting \textit{whether} driver is intending to takeover, if the driver does not have the intention, estimation of the time and quality of takeover will not be proceeded. Once the system indicates a high chance of taking over, driver's takeover time~(\textit{when}) and quality of takeover~(\textit{how}) will be anticipated. Despite the recent studies on prediction of each individual phase of the driver's takeover performance~\cite{du2020predicting,lotz2018predicting,deo2019looking}, the obtained accuracy of their models were insufficient for practical implementation. Herein, we focus on developing a more practical solution that not only applies to all phases of proper takeover behavior, but also significantly outperforms the state-of-the-art results prediction of driver's takeover intention~\cite{guo2019predictive}, times~\cite{lotz2018predicting}, and the quality~\cite{deo2019looking}. Furthermore, as we establish a novel approach on prediction of driver's takeover behavior, we offer our novel framework configurations, implementation details, and source code to the Human-Computer Interactions (HCI) community to reproduce our obtained results~\footnote{Website is anonymized for the review purpose.}.  

% our proposed approach is shown to outperform the binary prediction of \textit{whether} the driver will takeover or not.
% Once the system could estimate the binary action of takeover, it will reliably predict the time and the quality of the driver's response.


We envision that our robust estimation of driver's takeover time and the takeover quality can be integrated into an intelligent vehicle safety system both for (1) AVs that use driver state in optimizing transfer of control decisions along with motion planning, and (2) assistive technology such as future advanced driver assistance systems (ADAS). By integrating DeepTake framework into the monitoring systems of the AVs, the automated system knows the potential category of driver's takeover behavior and can adapt its driving behaviour to match the drivers need. In addition, our novel approach provides a promising new direction for modeling driver's takeover time to lessen the effect of general and fixed design of TORs which considers homogeneous takeover time for all drivers. Our framework allows the AV to constantly monitors the category of takeover time and takeover quality of a driver and gradually adjust to match the need for proper takeover control.


% ~(i.e., either to takeover or not) as well as the time required to perform the necessary set of actions before takeover.
% However, there will also be cases where the AV’s ability to drive safely and to monitor its performance, is
% 2019). However, there will also be cases where the AV’s ability to drive safely and to monitor its performance, is
% impaired.



Therefore, we outline contributions of this work as follows:
\begin{enumerate}
    % \item \textbf{Scenario design:} We account for multiple critical types of transition requests including planned transfer of control with explicit alarm~(true alarm), nuisance alarm~(false alarm) accompanied by silent failure~(no alarm) of the automated vehicle to practically predict driver takeover behavior.
    \item \textbf{Novel approach:} To the best of our knowledge, our proposed DeepTake method is the novel prediction of the driver's reaction time and quality of takeover using multimodal data. Our DNN-based framework shows the driver’s reaction time and quality of takeover can be predicted as early as 10-sec prior to the initiation of TORs. Therefore, the automated system could gradually adjust the TOR timing to the needs of driver.
    \item \textbf{Feature contribution:} We provide evidence how the magnitude of certain features affecting the category of takeover reaction time and takeover quality. It presents a novel insight into the optimum number of features per modal for future advancement of on-road takeover response prediction. Our findings can be used to filtrating features and capture the most important features for takeover  behavior classification
    
    % \item We show how the driver's action-related features which are passively collected from the wearable devices along with vehicle trajectories can be used in predictive modeling to increase the individual-sensitivity in a timely manner. It can be the primary step towards personalizing TORs.
    % \item \textbf{Outperformance:} While prior studies in prediction of RT is missing, we qualitatively show that our model outperforms the state-of-the-art results under binary action of takeover prediction~\cite{du2020predicting} and the quality of the takeover~\cite{deo2019looking}.
    % \item \textbf{Open Source and Reproducibility:} As we establish a novel approach on prediction of driver's RT, we provide our novel framework configurations, implementation details,~and source code to the Human-Computer Interactions (HCI) community to reproduce our obtained results.  
    % \item We discuss the implications of our work on the design of future neural net facilities, including using the information gathered to enhance the chance of the correct prediction of human behavior. This can be integrated into many current systems to improve the automation safety.
\end{enumerate}

% The remainder of this paper is organized as follows. We begin by reviewing the related works, and present the details of our methodology followed by modeling framework. Using the obtained data and developed framework, we investigate prediction of binary takeover action and multi-class classification of driver reaction time.


==> Sections/oldSections/MethodMotiv.tex <==


% What other studies have done?
% The majority of the studies have investigated the reaction time and and its relationship to the takeover quality in response to a TOR trigger. However, the recent automated accidents have shown that it is reasonable to expect that the automated system could fail to prompt TOR. Therefore, the automated system requires to constantly analyze the challenges and predict how the human's performance will be in an accurate and robust way using established sensor technology before triggering TORs.

AVs provide the underlying condition for users to have more free time to be engaged in NDRTs. Hence, their perception, and anticipation of incidents in the surrounding environment will be impaired until they have enough time to properly regain the situational awareness for a safe transition of control. A failure to reliably estimate the driver's cognitive and physical competence, situation awareness, and therefore takeover readiness before TOR, will cause anxiety to driver and potential tragic consequences to vehicle and its occupants. Thus, we propose DeepTake, an efficient multi-class DNN-based framework which accounts for continuous driver behavior monitoring by leveraging multimodal data including biometric sensors, NDRTs and engaged objects, vehicle dynamics, and subjective measurements, as illustrated in Figure~\ref{fig:llustrative}. 
It displays \textcolor{red}{our proposed DeepTake framework consisting of \textbf{four modules} dedicated to multimodal data collection, data preparation and feature extraction, DNN model, and classified takeover behavior outcomes.} Utilizing multimodal data fusion in our proposed DNN-based framework, helps more accurate and robust prediction of multiple phases of drivers’ takeover behavior~(\textit{where,when}, and~\textit{how}) than prior studies. DeepTake can help the automated system to adjust the TOR initiation to match drivers' takeover needs and ultimately help the driver to better prepared to safely navigate the incident for which the handover of control occurs. We explain each module of the DeepTake framework below.

\subsection{Multimodal data} \label{sec:Multimodal}
Figure~\ref{fig:llustrative} illustrates a user wearing biometric sensors showing changes in eye movement metrics accompanied by emotional responses while engaging with a ~\textcolor{red}{cellphone}. These non-intrusive, multimodal objective measurements detect driver's visual attention collected from eye-tracker, stress and anxiety through heart rate~(HR) and galvanic skin responses~(GSR). DeepTake framework incorporates wrist-type photoplethysmographic~(PPG) signals where its sensors' strap was wrapped around the participant's ring finger, while the GSR sensor straps was wrapped around the participant's index and middle finger~(See Figure~\ref{fig:llustrative}). Traditionally, driver status were only derived from the driving performance~(e.g., lateral and longitudinal control of the vehicle). However, since in the AVs drivers are no longer in control of the vehicle all the time, using wearable devices with big-data analytic can enable individualized measurement of driver's cognitive and physical states. Although we employed high-end sensors to precisely track driver's state changes, our intention were using physiological data as reliable features that future advancement of such system can be easily applied to real world applications. Below, we explain the subjective and objective multimodal measurements utilized in DeepTake framework indicating the drivers' visual attention, level of stress, and workload.


\subsubsection{Eye-tracker}
In automated vehicles, it is likely that drivers will engage with NDRTs. Eye-tracker captures eye-movement subsequent to shifting drivers visual attention before and after TOR. There is a high proven correlation between driver's eye movements and visual attention\cite{zeeb2015determines,wu2019assessing,alsaid2019moving}. In order to comprehend the attentiveness of driver to the surroundings environment before TOR, we acquired gaze coordinates, pupil diameters of each eye, fixation duration/sequence on the detected objects, and time to first fixation~(TTFF)~(see Table~\ref{tbl:data sources}). 
% One of the main components of eye-tracker is observation time which is calculated as the ratio between the fixation time and the time in which the object (e.g., pedestrian, truck, obstacle, etc.) appears in the visual frame. The smaller the ratio is, the less important (or not important at all) the object is to the driver or the driver failed to detect the object properly. 

\subsubsection{Heart Rate~(HR)} In a stressful driving context, variation of HR indicates the stress and affect situational awareness. DeepTake employs HR using photoplethysmographic~(PPG) signals recorded from
wearable Shimmer3 GSR+ device with a sampling frequency of 256Hz. PPG sensor monitors HR by emission of infrared light using LED into the body and measures the reflection back to estimate the blood flow. Unlike the electrocardiography~(ECG), PPG does not rely on the placement of metal electrodes on the participant's chest and can be found embedded in most smartwatches. Therefore, it not only provides us with the mobility required to gain uninterrupted information from the participants, but can also be practically employed as a result of requiring less intrusive body contact and maximized user experience. Fluctuation of heart rate in the time intervals between the nearby beats which occurs as a result of emotional factors can be measured by variability of heart rate~(HRV). HRV is the main parameter associated with detecting driver's workload~\cite{paxion2014mental}, driver's stress~\cite{dillen2020keep}, and driver's drowsiness~\cite{vicente2011detection}. In this study we extract features from HRV analysis for monitoring driver's readiness. 



\subsubsection{Galvanic Skin Responses~(GSR)} 
Another physiological data considered in this study is GSR, which simply indicates the conduction ability of the skin~\cite{dillen2020keep,nourbakhsh2012using}. As skin conductance is balanced by sweat secretion caused by sudomotor activity, any action accounting for muscle activation like stress can be objectified by GSR~\cite{braithwaite2013guide}. Therefore, in the context of driving any emotional arousal~(e.g. startle response, sudden fear, and stress), the magnitude of the electrical resistance of the skin decreases, while the conductance increases. Along with HR parameters, GSR has been proven as one of the most valid indicators of stress and workload of a drivers~\cite{dillen2020keep,foy2018mental,mehler2012sensitivity,radlmayr2014traffic}. Thus, it was used to monitor the objective stress level of drivers. 


\subsubsection{NASA-Task Load Index~(NASA-TLX)}
In order to complementing the objective measurements, we also use NASA-TLX as one of the most extensively exploited objective metrics for the measurement of driver's workload. We use NASA-TLX at the beginning of each trial to prevent participants become annoyed to rate their workload while driving. It provides ratings methods, on a scale with 21 gradations, across six critical domains for proper reaction in driving: mental demand, physical demand, temporal demand, performance, effort, and frustration.

\subsubsection{PSS-10.}
The 10‐item Perceived Stress Scale~(PSS‐10) is another subjective metric developed to measure perceived psychological stress or \textit{"stress-related components of unpredictable, uncontrollable, and overloading life events”}\cite{iseland2018exploratory} over the past 30 days. We only obtained this result once at the beginning of the driving session.


\subsubsection{Non-Driving Related Tasks~(NDRTs)}
AVs provide environments where drivers can interact with various NDRTs, such as reading books or using smartphones. These NDRTs play a crucial role in the acceptance of the automated vehicle. Each driving task, however, requires a certain level of visual, physical and cognitive demand. We selected the most common NDRTs herein to create realistic scenarios by which drivers would be most likely to engage in the AVs~\cite{gerber2020self,dogan2019effects}. These selected NRDTs include Reading, simple arithmetic problem solving questions, Browsing the Internet, and Conversation. These tasks were not only chosen to suit our experiments' setup~(see Figure~\ref{fig:simulator}), but also to follow the framework of difficulty level in flow theory~\cite{csikszentmihalyi1990flow}. The reading and arithmetic problem solving questions tasks have two main difficulty levels~(easy and medium adapted from\cite{nourbakhsh2012using} which reported strong correlation between the questions and physiological responses). 

\subsubsection{{Vehicle dynamics}}
From the vehicle dynamics data we capture the angle of the steering wheel, accelerator and brake pedals, distance from the neighbor lanes, distance to hazard, and finally the speed of the car. These features display the instantaneous driver's reactions in order to control the vehicle appropriately. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%===============================================
%%%%%%%%%%% Framework Graph %%%%%%%%%%% 

% \begin{figure*}[h!]
%   \centering
%   \includegraphics[width=5.2in]{Figures/NN_Structure_3.png}
%   \caption{The proposed DeepTake framework for the prediction of driver's takeover behavior based on a deep learning architecture. This framework includes four steps of multimodal data collection, data preparation and feature extraction, DNN model, and classified takeover behavior outcome. The input of the framework is the driver-related signals, vehicle dynamics information, subjective measurements, and the non driving-related tasks. The 10sec time window is selected where all the multimodal data is fused to feed into the DNN model. The output layer shows the three defined classes for the prediction of takeover(either takeover time or quality.)}
%   \label{fig: NN_Architecture}
% \end{figure*} 
%%%%%%%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Data preparation and feature extraction}\label{sec:Dataprep}
The wide range of a driver's action related features provides a better chance to draw insights into different types of driver's takeover behavior. However, the larger the number of features, the harder it is for the classification algorithm to build a comprehensive model from the obtained data, especially considering the smaller number of participants proportional to the number of features. Therefore, we initially prepare and extract the utmost features from all of the aforementioned modalities, then applied feature selection methods to reduce the number of features to a set that is representative of our data. 

As introduced in section~\ref{sec:Multimodal}, multimodal data including driver physiological signals from wearable devices, NDRTs, subjective measurements, and  vehicle dynamics were acquired. At this step of the DeepTake framework, the captured signals are filtered and meaningful features are extracted. This step aims to fuse all the multimodal data into a joint representation to feed into the next step of DNN model~(see Figure~\ref{fig: NN_Architecture}). Since DeepTake covers three \textcolor{red}{phases} of takeover behavior~(\textit{where, when,} and \textit{how}), the selected features need to expose all the three phases together to reliably guide the automated system about the driver's status. Therefore, features should be carefully and elaborately extracted, then selected. In order to do so, the primary essential step is finding an appropriate time window size. We applied fixed window method wherein the segmented windows will get the same labels as the original. Studies have found that 10 second is an adequate time budget for a driver to react properly\cite{walch2017car,zeeb2015determines}. Thus, we selected all of the following features over the 10sec fixed time window before the moment of takeover alarm. Within the segmented window, we preprocess and extract meaningful features from the physiological data. As the varying forms of signal used in DeepTake framework, we took the approach suitable for each individual signal. Our approach for identifying relevant and informative features is exploratory and based on previous research.


%===============================================
%%%%%%%%%%% List of Features %%%%%%%%%%% 

% Table for Features list
\vspace{-1mm}
\input{Tables/Features_list}
\vspace{-1mm}

%===============================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Feature Extraction}}

\paragraph{\textbf{PPG}}
As it is suggested by~\cite{singh2013comparative}, a min-max normalization was executed on PPG signals prior to pre-processing and feature extraction. We applied the min-max normalization on a 10second window of the baseline scenario as follows:

\begin{equation} \label{eq:Min-Max Normalization}
    S_{norm} =\frac{PPG_{raw} -\min(PPG_{raw})}{\max(PPG_{raw})-\min(PPG_{raw})}
\end{equation}

where $S_{norm}$ represents the normalized PPG signal. The normalized PPG signals were then filtered by applying a 2\nd order Butterworth high pass filter with a cut-off of 0.5Hz followed by a 1\st order Butterworth low pass filter with a cut-off frequency of 6Hz. The filtering procedure can be defined as: 

\begin{equation} \label{eq:Min-Max Normalization}
    S_p = f_{b}(S_{norm}, c_l, c_u)
\end{equation}

where $S_p$ represents the pre-processed signal and $c_l$ and $c_u$ show the lower and upper bound cutoffs, respectively. 
We used HeartPy, an open-source toolkit analyzing PPG data, for filtering and extracting the following features\cite{van2019heartpy}.

In this study we also extracted HRV assoiciated features from the preprocessed PPG signal~($S_p$)~and focused on the most common time-domain indices of HRV by which we could quantify the amount of HRV after receiving TOR. The extracted features used in this study include the standard deviation of normal beats~(SDNN), root mean square of successive differences between normal heartbeats~(RMSSD), and Percentage of the number of sequential normal beats differences that are over 50 ms~(pNN50). 

\paragraph{\textbf{GSR}}
For each TOR, GSR features were extracted from the part of the signal corresponding to 10second prior TOR. Important features extracted from skin conductance are 1)~the quantity of peaks and, 2)~the peak amplitude~\cite{manawadu2018tactical,nourbakhsh2012using}. A peak occurs when a subject gets a phasic response higher than the baseline of skin conductance~(the GSR signal contains phasic and tonic components and in this study we only use features extracted from the phasic component). The GSR peak amplitude is a measure of how far above the baseline the peak occurred. In other words, amplitude is the difference between the value of local maximum and the point the signal starts to rise.





\subsubsection{\textbf{Feature Selection}}\\
% feature selection
% and combination is another obstacle for accurate takeover behavior classification
To prepare the features for the DNN model, the sliding window of 10 sec was exploited to individual feature from each modality~(more details in sec~\ref{sec:Dataprep}. We included all of the data sources as we could possibly obtain and later acquired meaningful features from the multimodal data sources. To remove individual-dependency of the wearable signals, we normalized the features reported in Table~\ref{tbl:data sources} by Z-score normalization technique, except for PPG signals which we used min-max normalized. Finally, we reached more than 75 features, which is too many for the amount of data we had. Thus, we removed the features with no variation or a large amount of missing values~(more than 50\%). For features which passed this filtering process and still had missing values, their missing values were imputed with their mean values. We executed a correlation analysis on the feature set to identify features that are highly correlated with each other and therefore redundant with no discriminatory power to infer the driver's reaction time categories. This unbiased and compact set of features was selected using two feature selection methods: Least Absolute Shrinkage and Selection Operator~(LASSO) and Random Forests. We used LASSO to select a subset of features that are nearly independent and eliminate irrelevant variables to the driver's reaction time. LASSO performs well in selecting a stable set of features and tends to select one feature among highly correlated features, resulting in a reduction of features. Random Forests on the other hand rank all of the features based on their importance for the classification of reaction time. The overlapped features chosen by the two methods were utilized to develop the final classification model of reaction time.

Let the explanatory selected features be denoted as
$X= \{x_1, x_2,...,x_d\}$, where X is the set of pre-processed features we could pass X into our proposed neural net. The final features extracted and used in the model are shown in Table~\ref{tbl:data sources}. The intersection of the feature selection methods incorporated 35 features. Note that one-hot encoder was used to handle the categorical features which increase the number of columns for training the model.

% To prepare the data for the CNN architecture, the sliding win- dow strategy was applied to each low level feature from each modality. Using sliding window strategy, the signals are segmented into a fixed window size. The segmented windows are the new training data and will get the same labels as the original trials
\subsection{Target Labeling}
We used features listed in Table~\ref{tbl:data sources} to feed to the DNN model to predict driver takeover behavior including \textit{intention}, \textit{time} and \textit{quality}. Previous studies defined the labels objectively through asking multiple humans to watch and rate the driver's performance~\cite{deo2019looking,du2020predicting}.
However, the key for practical application is subjectively selecting thresholds for acquiring the target labels. Thus, we define the takeover intention, time and quality labels for DeepTake framework as follow.

\subsubsection{Takeover Intention}
The takeover intention is a binary action of whether the driver is willing to takeover or not. Therefore, once the driver initiates the action of resuming the control by pressing the two buttons mounted on the steering wheel~(see Figure~\ref{fig:simulator})the multimodal data are labeled as \textit{takeover}, otherwise \textit{not-takeover}.

\subsubsection{Takeover Time}
While driving the AVs, the system initiates the TOR ($t_{alarm}$), drivers should regain the situational awareness and assess the scene for the necessity of taking over. If the driver quickly observes the situation and decides that the current lane is not safe, she is obligated to maneuver the vehicle safely. The moment of taking over or the starting time of manually controlling the vehicle is defined as $t_{takeover}$~\cite{sadeghian2018feel,gold2015utilization}. The $t_{takeover}$ is defined as the first contact with the steering wheel/pedals~\cite{zeeb2015determines} or pressing the takeover buttons~\cite{kim2017takeover}. In our driving simulator environment, once the participant assumes control by simultaneously pressing two assigned buttons on the steering wheel~(more details in sec~\ref{sec:Procedure}). Thus, the value of \textit{reaction time~(RT)} was calculated as:
\begin{equation} \label{eq: reaction time}
    \centering
    \textit{RT} = t_{takeover} - t_{alarm}
\end{equation}

The time interval between the TOR and the completion of the transition to manual driving is RT~(see Figure~\ref{fig:Scenario}). Subsequently, with the intention of creating multi-classes of reaction time, we modified reaction time into \textit{three} and \textit{five classes}. The  thresholds for each class of RT complies the existing lines of research in pre-defined i\textsuperscript{th} percentile of RT~\cite{coley2009driver} where three-class of RT is thereby classified as: low-~($RT <2.6sec$ ), medium-~( $2.6sec \leq RT \leq 6.1sec$), and high-~($6.1sec <~RT$) reaction time. This led us to even narrower five-class classifications of reaction time in which each class is defined as: lowest-~(RT < $1.5sec$), low-~($1.5sec \leq RT < 2.6sec$), medium-~($2.6sec \leq RT < 4.7sec$), high-~($4.7sec \leq RT \leq 6.1sec$), highest-~($6.1sec < ~RT$).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Takeover Quality}
Driver reaction time is how prepared the driver is to take the control, whereas the quality is defined by the occurrence of driving errors such as lane exceedances, insufficient securing or inadequate speed. Thus, the takeover quality is measuring how safe the driver's maneuver the control of the car. The performance metrics for evaluating this matter is either based on braking or steering performance~\cite{happee2017take}.In this study, we apply the latter metric where variability of vehicle position is used to infer how well the driver takeover.  low-~($position <3.5m$ ), medium-~( $3.5m \leq position \leq 7m$), and high-~($7m <~position$) takeover quality.

\subsubsection{Fusion} Due to the varying modalitis collected in this study and signal complexity driven by underlying preprocessing and feature extraction, extracted features~(Table.\ref{tbl:data sources}) are combined into one vector to use into the DNN model.


%%%%%% Driving Simulator %%%%%%%%%%%%%%%%
% \textcolor{blue}{
% Driver takeover and reaction time was studied with the use of a driving simulator. The main advantage of utilizing any driving simulator is not only creating all possible driving scenarios which drivers may or may not encounter daily, but also collecting vehicle information such as speed, lateral and longitudinal positions which may not be easily feasible in the field. Besides, we could safely collect subjective detailed measurements of drivers through various surveys. All the aforementioned benefits can be used as the features for developing a robust framework for predicting driver reaction time.}







% \textcolor{blue}{
% %-------------------
% % WHY DNN or ML?
% Automated systems tend to minimize the intervention rate but they are still unequipped to tackle several sudden events~\cite{favaro2018autonomous} and therefore rely on human's abilities to assist~\cite{seppelt2019keeping}. Nevertheless, as the automated systems alter the driver's performance, they have a greater difficulty in safely controlling the automated vehicle, due to substantially losing situational awareness~\cite{merat2014transition}. 
% % Given adequate time, however, their performance improves~\cite{gold2018modeling}.
% While automation behavior can be predicted to some \todo{extent}, human behavior is inherently stochastic and conditioned to a determined situation. This makes predicting human behavior difficult and crucial to combat. Fortunately, the recent rapid advancement of DNN techniques equipped with enough data shows stellar reliability for modelling human behavior~\cite{kim2020fundamentals}.
% Much research has focused on understanding different aspects of the reaction time such as the time gap needed for drivers to react properly and statistical analysis of drivers reaction time. However, a few studies have focused on providing a cohesive, holistic framework by which the system could decide the human driver is prepared enough to safely takeover. Our framework provides the fundamentals for a system to reliably predict the drivers reaction time and quality of takeover based on their performance history through using Deep Learning.}



% \textcolor{red}{Why NDRTs}
% Conditionally automated driving and the engagement in NDRTs represents a novel situation for a driver, in which drivers have more free time to the task they desire to. In such situation, the future of mobility will depend on the constructive collaboration between human and the automated system. In this study we aim to provide the opportunity not to limit driver access to NDRTs, but to provide enough time for driver to adjust the situation to takeover when it's needed. Although the in-lab setup was used due to the fact that it is nearly impossible to collect enough driver reaction time data before dangerous events with the conventional in-car data collection protocol and safety concern,the presented framework can impact on how humans would interact with automated vehicle. The in-lab setting provided some of the most common tasks which may drivers will interaction with while riding.

% \textcolor{red}{BigPicture:}
% When the automated system evaluates whether a non-controllable event could happen and the situation might be safety-critical it will assess the situation of driver to take-over the control. To assess the driver status, there are two factors that a system needs to evaluate before relinquishing the control in a timely manner: 1) Driver’s reaction time, 2) Quality of takeover
% Driver reaction time is how prepared the driver is to take the control where as the quality is defined by the occurrence of driving errors such as lane exceedances, insufficient securing or inadequate speed. The correct and reliable judgment of driver status could be life-saving which lead to higher performance to be near perfect.  \\



==> Sections/oldSections/Modeling.tex <==

This section presents the multimodal DNN architecture of DeepTake framework. Figure~\ref{fig: NN_Architecture} shows the steps of DeepTake framework for the classification of multi-class takeover behavior. We described how the signals were processed followed by features extraction in Sec.\ref{sec:Dataprep}. In this step, we fuse the extracted multimodal features to build a DNN model to detect binary class of driver's takeover intention~(whether), three classes of takeover time~(when), and three classes of takeover quality~(how). 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}[t!]
% \caption{Train a neural network with mini-batch stochastic gradient descent}
% \begin{algorithmic}[1] \label{alg:NN}
% \STATE   $X,y \gets  Preprocess (x,y)$
% \STATE  Upsampling~$(X,y)$   
% \STATE initialize($net$)
% %\STATE Split~(train,test)
%     \FOR{ epoch $= 1,...,K $}
%         \FOR{ batch = 1,...,b}
%         \STATE validation = $0.1$
%               \STATE  $z \gets$ forward$(net, X)$
%               \STATE $ \ell \gets$ loss$(z, y)$
%               \STATE $grad \gets$ backward($\ell$)
%               \STATE update($net, grad$)
%         \ENDFOR
%     \ENDFOR
% \end{algorithmic}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Classification}\label{sec:classifications}
In order to implement a framework in the real world, we should first and foremost assure the safety of the users by using methods with the highest reliability. Prediction of each individual phase of takeover behavior, intention, time and quality, has been studied but they have not been able to achieve a relatively high accuracy. Comparing the results of takeover intention binary classification,  provides the confidence in our selected features to tackle a more challenging problem of multi-class classification of takeover time and quality using the same features. We applied our selected features into multiple machine learning algorithms to compare their performances in all three phases of takeover. Our process of choosing the learning algorithms is an exploratory task with trials and tests of multiple off-the-shelf algorithms~(see Table~\ref{tbl:results comparison}) and choosing those that perform the best. We evaluate the performance of Logistic Regression, Gradient Boosting, Random Forest,  Bayesian Network, Adaptive Boosting~(Adaboost), and Regularized Greedy Forest~(RGF). RGF with Adaboost provide the best performance according to our evaluation criteria explained below.


\subsubsection{Neural Network Architecture}
DeepTake utilizes feed-forward DNN with mini-batch stochastic gradient descent. This DNN structure begins with an input layer to match the input features and each layer receives the input values from the prior layer and outputs to the next one~(see Figure~\ref{fig: NN_Architecture}). DNN provides the flexibility to process the inputs independently so that it fits feature complexity. The DNN in this study includes three hidden layers with 23, 14, and 8 \textit{ReLu} units respectively in hidden layers. As the main purpose of this paper is to develop a model for multi-class classification of driver takeover behavior, the output layer of DNN consists of three \textit{Softmax} units representing three takeover time and quality classes~(low-, medium-, and high-). Therefore, our implemented DNN uses ReLU~(equation \ref{eq:Relu funciton}) as an activation function in each hidden layer and uses the Softmax~(equation \ref{eq:Softmax funciton}) function as the classification function at the last layer of the network.

\begin{equation} \label{eq:Relu funciton}
    f(x) = max(0,x)
\end{equation}

\begin{equation} \label{eq:Softmax funciton}
    \sigma(z)_j = \frac{e^{z_j}}{\sum_{k=1}^k e^{z_k}} \\~, \forall j \in\{1,...,k\}
\end{equation}

We used Softmax cross-entropy loss with an Adam optimizer with a learning rate of 0.001 to update our parameters and trained our DNN model over 400 epochs. In each iteration, we randomly sampled a batch of data in order to compute the gradients with a batch size of 30~($b=30$). Once the gradients were computed, the initiated parameters got updated. It automatically stops after 400 passes through the dataset. The early stopping method throughout the training procedure prevented overfitting.




==> Sections/oldSections/Results.tex <==
%%%%%%%%%%% Accuracy Vs Loss %%%%%%%%%%% 
\begin{figure}[t!]
\centering
   \includegraphics[width=\textwidth]{Figures/ROC_3RT_Quality.png}
   \caption{a) The ROC curve of six machine learning algorithms employed for classification of takeover. ROC curve shows the average performance of each classifier and the shadowed areas represent the 95\% confidence interval.  The AUC value of 0.5 refers to a random classifier. In the legend, the AUC associated with each classifier is shown. b)\textcolor{red}{change the caption}}
   \label{fig:ROC}
\end{figure} 
%%%%%%


%%%%%%%%%%% Table for model comparison %%%%%%%%%%%%%%%%%%%%%%
\vspace{1mm}
\input{Tables/Model_Comparision}
\vspace{0.1mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As the prediction of driver reaction time is contingent upon the driver's decision to take over from the autonomous systems after receiving TOR, we had to predict whether drivers were able to take over or not. Although takeover prediction has been recently studied~\cite{du2020predicting,braunagel2017ready}, it still needs an extensive improvement to be practical and integrated into an automated system. Our extracted features contributed to a higher prediction accuracy in the binary classification of takeover. The results show~(Table~\ref{tbl:results comparison}) that RGF attains the highest accuracy and weighted F1 score~(92\% and 89\%) followed by AdaBoost~(88\% and 88\%) and Logistic Regression~(77\% and 88\%). Moreover, ROC was applied in order to better evaluate each of the classifiers. Figure~\ref{fig:ROC} shows ROC curves and AUC values for all six machine learning models to infer the binary action of takeover. RGF showed the best classification performance with an AUC of 0.94. Similar to accuracy level, AdaBoost had a slightly lower performance with an AUC= 0.91. The AUC values provided in Figure~\ref{fig:ROC} can be interpreted as the probability of  correctly classifying the driver takeover into the candidate category is higher than randomly selecting takeover or not-takeover~(red line in Figure~\ref{fig:ROC}). Table~\ref{tbl:results comparison} together with the results obtained from the AUC in Figure~\ref{fig:ROC} ensure that our selected features with the right classifier surpass the takeover prediction of previous studies. 

Therefore, a better performance in takeover detection achieved through the machine learning algorithms~(see Table \ref{tbl:results comparison}) led us to a multi-class prediction of driver reaction time. As some of the machine learning algorithms attained high accuracy in binary classification of takeover, their performances along with our developed DNN in classifying multi-class classification of reaction time would show the robustness of the model.

For the training of our DNN, 70\% of the data was used and the rest was assigned equally for the testing and validation. As explained in \textcolor{red}{Algorithm~\ref{alg:NN}}, in order to satisfy the imbalanced data in each category, data in the minority classes were required to be upsampled. Due to the size of the dataset, the processing of each epoch lasted 570 seconds, that is, in comparison with the other tests, the computational effort was increased to generate a more robust model.


%%%%%%%%%%% Accuracy Vs Loss %%%%%%%%%%% 
\begin{figure*}[t!]
\centering
   \includegraphics[width=5.5in]{Figures/Accuracy_vs_Loss.pdf}
   \caption{The left figure shows the accuracy result of training and test sets for 400 epochs whereas the right figure indicates the loss for our DNN model on prediction of three class driver's reaction time.}
   \label{fig:Model_Accuracy_vs_Loss}
\end{figure*} 
%%%%%%

Table~\ref{tbl:results comparison} compares our DNN model with other classifier algorithms. It is evident that our DNN outperforms all of the classic algorithms. In three-class classification of reaction time~(low,~mid,~high), the DNN model achieves a weighted-F1 score of 0.87, thereby achieving the best performance on this task by a substantially better accuracy result of 92.3\%. As shown in Figure~\ref{fig:Model_Accuracy_vs_Loss}, DNN gained a high accuracy for both the learning and testing sets. However, the model did not significantly improve and stayed around 92\% accuracy after the epoch 250. Among the classifiers, though, RGF and AdaBoost still performed better~(73.4\% and 64.1\%).

In the five-class classification of reaction time, the results on the validation set show that DNN model also outperformed~(around 12\% more than RGF and 115\% better than RandomForest) the standard machine learning classifiers with respect to weighted F1- score and accuracy. As shown in Table~\ref{tbl:results comparison}, the performance of each model varied regardless of the number of classes. But, similar to three-class classification, the RGF model achieved the best performance~(66.4\% accuracy) on the five-class distinction of reaction time among the six machine learning algorithms. The other algorithms achieved lower performance than the RGF model.


%%%%%%%%%%% Confusion Matrix 3_Class %%%%%%%%%%% 
\begin{figure}[h!]
\centering
  \includegraphics[width=0.48\textwidth]{Figures/CM_ThreeCL_RT.png}
  \caption{Confusion matrix for the prediction of three classes of driver's takeover time.}
  \label{fig:CM-ThreeClass}
\end{figure}
%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 

To capture a better view of the performance of our DNN model on reaction time prediction, we computed the confusion matrix for each multi-class classification problem. Figure~\ref{fig:CM-ThreeClass} displays the performance of our DNN model as the best classifier of three-class reaction time. As the diagonal shows the number of correctly classified, it can be seen that the misclassification in each class is small. The lowest true positive number is achieved by the medium reaction time class. Also, marginal misclassifications are found in the 1\%-2\% of the low and high reaction time label. Overall, the DNN model obtains good performances in correctly classifying the three-class reaction time.

Figure~\ref{fig:CM-FiveClass} represents the performance of DNN on classifying the five-class reaction time. Although DNN was not as distinctive in five-class classification as in the three-class, it still achieved satisfactory results. Lowest, low and medium reaction times are the top three pairs that were the most frequently misclassified by the DNN algorithm. The reason might be that the selected features do not have the required distinctive characteristics to perfectly divide the low and medium reaction times. In each class, however, it could still distinguish between four other classes with an average of 70\%. 


%%%%%%%%%%% Confusion Matrix 5_Class %%%%%%%%%%% 
\begin{figure}[h!]
\centering
  \includegraphics[width=0.48\textwidth]{Figures/CM_FiveCL_RT.png}
  \caption{Confusion matrix for the prediction of five classes of driver takeover time.}
  \label{fig:CM-FiveClass}
\end{figure}
%%%%%%%%%%% %%%%%%%%%%% %%%%%%%%%%% 


\subsection{\textcolor{red}{Takeover Quality w.r.t position}}


==> Tables/TOR_Modalities.tex <==
\begin{table}[h!]
\small\addtolength{\tabcolsep}{-5pt}
  \begin{center}
    \caption{Takeover request modalities}
    \label{tbl:TOR_Modalities}
    \begin{tabular}{l| p{60mm}}
      \toprule % <-- Toprule here
      \textbf{Types of TOR} &
      \textbf{Explanation}\\
      \hline \hline
      False Alarm~(FA)  & Takeover request in the situation where it is safely managed or wrongly recognized \cite{naujoks2014effect}\\
     \hline
      No Alarm~(NA)  & Not initiating Takeover request in the situation that is needed\\
      \hline
      True Alarm~(TA) & Correctly initiating Takeover request in the situation that is needed\\
     \bottomrule % <-- Bottomrule here
    \end{tabular}
%{\scriptsize 1: \textit{Number of repetitions for each type of alarm.}}
  \end{center}
\end{table}
